Deep Unsupervised Cardinality Estimation

Cardinality estimation has long been grounded in statistical tools for density estimation. To capture the rich multivariate distributions of relational tables, we propose the use of a new type of high-capacity statistical model: deep autoregressive models. However, direct application of these models leads to a limited estimator that is prohibitively expensive to evaluate for range or wildcard predicates. To produce a truly usable estimator, we develop a Monte Carlo integration scheme on top of autoregressive models that can efficiently handle range queries with dozens of dimensions or more. Like classical synopses, our estimator summarizes the data without supervision. Unlike previous solutions, we approximate the joint data distribution without any independence assumptions. Evaluated on real-world datasets and compared against real systems and dominant families of techniques, our estimator achieves single-digit multiplicative error at tail, an up to 90$\times$ accuracy improvement over the second best method, and is space- and runtime-efficient.

==> abstract-v0.tex <==
Selectivity estimators traditionally make the hard tradeoff between accuracy and
storage/construction efficiency by either placing restrictive column
independence assumptions (statistical synopses), or avoiding modeling the data
altogether (sampling and query-driven techniques).  This paper argues for dispensing with
this tradeoff entirely.
By placing no independence assumptions
and approximating the joint data distribution in its full
form---a goal previously thought intractable---we show that significant benefits
in accuracy, efficiency, and simplicity can be
obtained
at the same time.

Key to enabling our estimator is the use of high-capacity yet compact deep neural
net-based likelihood models.  However, a direct adaptation of these models to
selectivity estimation yields limited capability: conjunctions of range
predicates can be prohibitively expensive to estimate.  To make them truly practical, we
propose an efficient Monte Carlo integration scheme to support range queries
with even up to more than a dozen filters.  Evaluation on several real-world
datasets and comparisons against real systems and dominant families of
estimators show that our direct joint approximation approach can achieve
single-digit multiplicative error at tail, a
$20{-}100\times$ accuracy improvement over the next best method,
while remaining practically efficient.

==> graveyard.tex <==

\section{Graveyard...}
\subsubsection{Trading Off Accuracy for Latency}

The latency overhead of \sys scales linearly with the number of progressive sample paths used. Hence, when higher accuracy estimates are required, more paths can be taken.

Nugget: all other baselines are flat lines and \sys is the only estimator with a roofline-like shape (slanted then flat).  Interesting capability that no one else can do.

Also kind of shows the variance of psampling.


\subsubsection{Results on \imdb}
\zongheng{TODO: think about breaking this experiment into different parts.}
Is \sys still effective when asked to learn a joined relation?  As discussed in \secref{sec:construction-joins}, in principle learning a likelihood model on a join product is not technically different from learning on a base relation.  We nevertheless include this experiment as a proof-of-concept.  Here we train \sys on the \imdb dataset (Table~\ref{table:datasets}) which is the joined result of 4 base tables.

Table~\ref{table:imdb-weak-correlation} shows the estimation quality.  The trained model has a 0.65 bits  of KL-divergence between model and data.  We run 2,000 queries with a filter on each column where {\sf product\_year} is eligible for a range predicate.
%21.540-20.885

% c67: logs/imdb101M-2000queries-allFiltered-rangeOnProductionYear-61.8MB-model21.540-data20.885.csv
\begin{table}[hp]\centering \small%
\begin{tabular}{@{} l l l l l | l @{}} \toprule
  & \sc{Median} & \sc{95th} & \sc{99th} & \sc{Max} & {\sc  Latency}  \\ \midrule
{\sf Indep} & 1.37 & 10.00 & 31.00 & 113 & 3947ms\\
{\sf Sample} & 1.38 & 47.00 & 116 & 222 & 2149ms \\
\sys-1000 & 1.37 & 6.75 & 21.50 & 58 & 44ms \\
{\sys}-enum & 1.37 & 6.67 & 21.50 & 58 & 25ms \\
\bottomrule
\end{tabular}
\vspace{0.25em}
\caption{\small {
{\bf Estimation errors on the weakly correlated \imdb.}  \sys and {\sf Sample} consume 1.6\% of space.  Max latency is shown.
}\label{table:imdb-weak-correlation}
}
\end{table}

As discussed in \secref{sec:construction-joins}, in principle a streaming k-way join algorithm is the ideal choice for data ingestion, although the joined relation we consider now is small enough to be fully materialize first.   Similar treatment was adopted in prior work~\cite{kiefer2017estimating}. We defer the design of a streaming join ingestion scheme to future work.  However, this experiment does illustrate a few new points not highlighted in the \dmv or \conviva results:

First, our embedding encoding/decoding scheme is highly beneficial for columns with a huge domain size (\secref{sec:encoding-decoding}).  \imdb contains {\sf keyword\_id} which has a domain of 119K distinct values.  Here, \sys uses a 128-dimensional embedding vector for each distinct value and substantially cuts down the compute cost.  (The alternative one-hot decoding would involve a matrix multiply with a weight matrix $\mathbb{R}^{119219 \times h}$ where $h$ is the number of hidden units, usually chosen between 256 to 2048.  Namely, it would be computationally too expensive.)  This scheme is especially crucial if high-domain ID columns are involved.

Second, this experiment shows that \sys is effective even on a table with weak inter-column correlation.   We computed the Pearson correlation between each pair of columns in \imdb: the (absolute) correlation values range from a minimum of 0.008 to
a maximum of 0.128, indicating weak correlation.  In other words, \sys is highly accurate even on datasets where traditional independence assumption would mostly hold.


\begin{table*}[t!]\centering %\small%
\ra{1.4}
\begin{tabularx}{\textwidth}{l c c c c X } \toprule
% \begin{tabular}{@{} l c c c c p{4cm} @{}} \toprule
% & \textbf{\textit{Point density?}}	& \textbf{\textit{Conditionals?}}	& \textbf{\textit{Sample?}}	& \textbf{\textit{Range density?}}	& \textbf{\textit{Potential tasks}} \\
% & \textit{Point density?}	& \textit{Conditionals?}	& \textit{Sample?}	& \textit{Range density?}	& \textit{Potential tasks} \\
& \textbf{Point density?}	& \textbf{Conditionals?}	& \textbf{Sample?}	& \textbf{Range density?}	& \textbf{Fits selectivity estimation?} \\
\midrule
% Latent variable models (VAE) & \checkmark &\ding{53}& Y, fast & N & AQP, compression \\
GAN & \xmark & \xmark & \checkmark & \xmark & \xmark  \\
Latent variable (VAE) & \checkmark & \xmark & \checkmark (fast) & \xmark & \xmark \\
Normalizing flows	& \checkmark &  \xmark & 	\checkmark (fast) & 	\xmark & 	\xmark \\
Autoregressive	& \checkmark (high fidelity)	&  \checkmark & 	\checkmark  & 	\xmark & 	  Equality filters only \\
% \midrule
Autoregressive {\tt +} \sys & 	\checkmark (high fidelity) & \checkmark & \checkmark 	& \checkmark	& Wide support: range/equality filters; continuous/categorical; small/large domain size\\
\bottomrule
\end{tabularx}
% \end{tabular}
\vspace{0.25em}
\caption{{Generative models with different capabilities, and how they might fit the selectivity estimation task.}\label{table:likelihood-models}}
\end{table*}

\begin{table*}[t!]\centering \small%
\ra{1.3}
\begin{tabular}{@{} l l l l l l l l l l l l l l l l @{}} \toprule
\textbf{Estimator} && \multicolumn{4}{c}{\bf High ($(2\%, 100\%]$)}  & & \multicolumn{4}{c}{\bf Medium ($(0.5\%, 2\%]$)} & & \multicolumn{4}{c}{\bf Low ($\leq 0.5\%$)} \\
  % \cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12}
  && Median  & 95th & 99th & Max  && Median  & 95th & 99th & Max && Median  & 95th & 99th & Max\\ \midrule
{\sf SQLServ} && ? & ? & ? & ?
    && ? & ? & ? & ?
    && ? & ? & ? & ? \\
{\sf Sample($2.5\%$)} && 1.01 & 1.05 & 1.06 & 1.09
    && 1.04 & 1.11 & 1.15 & 1.22
    && 1.17 & 12.00 & 43.00 & 113 \\
{\sf KDE} && ? & ? & ? & ?
    && ? & ? & ? & ?
    && ? & ? & ? & ? \\
{\sf MSCN} && ? & ? & ? & ?
    && ? & ? & ? & ?
    && ? & ? & ? & ? \\
    \midrule
 % 'models/made-conviva25-model22.485-data18.489-512_512-ioEmbed-emb64-100epochs.pt'
 \sys: 2.5\%, 4 bits gap &&  & &  &
    &&  &  & &
    &&  & & & \\
 1K prog. samples && 1.04 & 1.23 & 1.38 & 1.61
    && 1.12 & 1.54 & 1.99 & 2.17
    && 1.27 & 39.73 & 579.25 & 2730 \\
 2K prog. samples
%  (0.2s)
 && 1.03 & 1.17 & 1.27 & 1.45
    && 1.10 & 1.38 & 1.57 & 1.69
    &&  1.21 & 13.25 & 240.65 & 1889 \\
 6K prog. samples && 1.02 & 1.12 & 1.18 & 1.33
    && 1.06 & 1.22 & 1.31 & 1.79
    && 1.15 & 4.81 & 46.86 & 443 \\
 10K prog. samples && 1.02 & 1.11 & 1.19 & 1.29
    && 1.06 & 1.18 & 1.26 & 1.62
    && 1.14 & 2.54 & 14.65 & 54 \\
 50K prog. samples
%  (1s)
 && 1.02 & 1.05 & 1.08 & 1.16
    && 1.04 & 1.14 & 1.17 & 1.19
    && 1.09 & 1.81 & 3.76 & 35 \\
\midrule
% 'models/conviva25-18.2MB-model21.596-data18.489-relNet-inferNet256-emb128-inferDirectIo-sumPool-1orders-embedInembedOut-doScaleEmbWhenDot-doLN-100epochs.pt'
% logs/conviva25-2000queries-unif4_11-rangeOnGeq10-psample1k_2k_6k_10k-model18.2MB_21.596.csv
 \sys2: 7\%, 3.1 bits gap &&  & &  &
    &&  &  & &
    &&  & & & \\
1K prog. samples
% (370ms)
&& 1.04 & 1.24 & 1.40 & 1.61
    && 1.10 & 1.51 & 1.85 & 2.70
    && 1.29 & 35.70 & 214.67 & 1362 \\
2K prog. samples
% (370ms)
&& 1.03 & 1.15 & 1.25 & 1.36
    && 1.09 & 1.40 & 1.63 & 1.85
    && 1.19 & 13.17 & 151.99 & 1943  \\
6K prog. samples
% (400ms)
&& 1.03 & 1.11 & 1.17 & 1.23
    && 1.06 & 1.22 & 1.33 & 1.42
    && 1.13 & 3.29 & 41.00 & 129 \\
10K prog. samples
% (600ms)
&& 1.02 & 1.11 & 1.16 & 1.19
    && 1.05 & 1.19 & 1.26 & 1.34
    && 1.12 & 2.70 & 14.00 & 142 \\
% latency in this table are median
\bottomrule
\end{tabular}
\vspace{0.25em}
\caption{\small{\textbf{Estimation errors on the Conviva-25 dataset} (25 columns).  Workload contains 2,000 queries where the number of filters is drawn from $\text{Unif}[4,11]$. \sys uses 2.5\% of space and has a gap of 4 bits/tuple to data; \sys2: $7\%$ of space, 3.1 bits/tuple gap.}
}}
\end{table*}


% logs/conviva22-2000queries-unif4_11-rangeOnGeq10-sample9_sample18.csv
\begin{table*}[t!]\centering \small%
\ra{1.3}
\begin{tabular}{@{} l l l l l l l l l l l l l l l l @{}} \toprule
\textbf{Estimator} && \multicolumn{4}{c}{\bf High ($(2\%, 100\%]$)}  & & \multicolumn{4}{c}{\bf Medium ($(0.5\%, 2\%]$)} & & \multicolumn{4}{c}{\bf Low ($\leq 0.5\%$)} \\
  % \cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12}
  && Median  & 95th & 99th & Max  && Median  & 95th & 99th & Max && Median  & 95th & 99th & Max\\ \midrule
  % latency in this table are max
{\sf Sample(9\%)}
% (390ms)
&& 1.00 & 1.02 & 1.03 & 1.05
    &&  1.02 & 1.05 & 1.07 & 1.10
    &&   1.10 & 5.00 & 13.91 & 39  \\
{\sf Sample(18\%)}
% (670ms)
&& 1.00 & 1.02 & 1.02 & 1.04
    && 1.01 & 1.04 & 1.05 & 1.07
    && 1.06 & 2.40 & 6.00 & 8 \\
    \midrule
% conviva22-20.8MB-model21.361-data18.190-relNet-inferNet128_128_128-emb128-inferDirectIo-maxPool-1orders-100epochs.pt
 \sys2: 9\%, 3.1 bits gap &&  & &  &
    &&  &  & &
    &&  & & & \\
1K prog. samples && ? & ? & ? & ?
    && ? & ? & ? & ?
    && ? & ? & ? & ? \\
2K prog. samples && ? & ? & ? & ?
    && ? & ? & ? & ?
    && ? & ? & ? & ? \\
    \midrule

% conviva22-42.1MB-model19.258-data18.190-relNet-inferNet1024_1024_1024-emb256-noinferDirectIo-sumPool-1orders-embedInembedOut-3tied-100epochs.pt
 \sys2: 18\%, 1.07 bits gap &&  & &  &
    &&  &  & &
    &&  & & & \\
1K prog. samples && 1.04 & 1.20 & 1.30 & 1.45
    && 1.10 & 1.53 & 1.98 & 2.85
    && 1.27 & 55.11 & 309.37 & 1724 \\
2K prog. samples && 1.03 & 1.14 & 1.25 & 1.45
    && 1.07 & 1.29 & 1.46 & 2.07
    && 1.19 & 23.25 & 276.87 & 773 \\
    \midrule
% conviva22-231.3MB-model18.700-data18.190-relNet-inferNet1024_1024_1024-emb256-noinferDirectIo-sumPool-1orders-embedInembedOut-100epochs.pt

 \sys2: 100\%, 0.5 bits gap &&  & &  &
    &&  &  & &
    &&  & & & \\
1K prog. samples
% (390ms)
&&  1.03 & 1.19 & 1.39 & 1.88
    &&  1.09 & 1.45 & 1.79 & 2.68
    &&  1.26 & 99.75 & 736.37 & 1975\\
2K prog. samples
% (670ms)
&& 1.02 & 1.14 & 1.22 & 1.40
    && 1.07 & 1.43 & 1.56 & 1.78
    && 1.18 & 17.55 & 190.73 & 1332 \\
\bottomrule
\end{tabular}
\vspace{0.25em}
\caption{\small{\textbf{Estimation errors on the Conviva-22 dataset} (22 columns). Workload contains 2,000 queries where the number of filters is drawn from $\text{Unif}[4,11]$.   \sys operates on a smooth trade-off curve between space/latency and estimation quality.}
}}
\end{table*}


==> intro-apr30MorningEdits.tex <==
\section{Introduction}
% what problem, why important, is it unresolved
Estimating the selectivity of a SQL predicate
% is essential
is a core primitive
in query optimization~\cite{systemr}, approximate query processing~\cite{blinkdb}, and performance profiling~\cite{akdere2012learning}.  The main task is to estimate the fraction of a relation that
satisfies a predicate, without actual execution.
% Despite its crucial importance, the problem is widely understood to be unresolved.
Despite its importance, there is wide agreement that the problem is
still unsolved~\cite{leis2015good,leis2018query,reopt}.
Open-source and commercial DBMSes
routinely produce up to $10^4{-}10^8\times$ estimation errors, depending on
the number of attributes, compared to the ground truth~\cite{leis2015good}.

% why is the problem hard
% The problem's hardness comes from the fact that estimators are tasked with condensing information
The fundamental difficulty of selectivity estimation comes from condensing information
about data into summaries~\cite{space_synopsis}.  The predominant approach in database systems today
is to collect single-column summaries (e.g., histograms and sketches) and to
combine these coarse-grained models assuming column independence.  This
represents one extreme, where the summaries are fast to construct and cheap to
store, but compounding errors occur due to the coarse information and over-simplified
independence assumptions.
% On the other extreme, when given access to a complete
% description about data, e.g., the true {\em joint data distribution}, selectivity
% ``estimates'' would be perfect albeit at the cost of intractable construction and
% storage.
On the other end of the spectrum, when given the {\em joint data distribution} of
a relation
(the frequency of each unique tuple normalized by the relation's cardinality),
perfect selectivity ``estimates'' can be read off or computed by integration from the distribution. However,
the {\em joint} is intractable to compute or store for all but the tiniest datasets.
% We show that the intractable joint data distribution of a relation,
 % can be approximated by deep likelihood models
% to a high degree of fidelity while offering compactness, functionality, and
% runtime efficiency.
Thus, traditional selectivity estimators are faced with the hard
tradeoff between the amount of information captured
%(more means better accuracy)
and the cost to construct, store, and query the summary.
%(the more information, the higher the costs).

\begin{figure}[t]
% \centering
\includegraphics[width=0.9\columnwidth]{plots/sol-space.pdf}
% \vspace{.1in}
\caption{Approximating the joint data distribution in full, \sys enjoys high space efficiency and estimation accuracy.\label{fig:teaser}}
\vspace{-.1in}
\end{figure}

% We argue that learning-based approaches can provide access to better points in
% this trade-off space (Figure~\ref{fig:teaser}).
% what enabled our attack
% We argue there is hope for dispensing with this tradeoff entirely.
An accurate and compact {\em joint approximation} would largely dispense with this
tradeoff (Figure~\ref{fig:teaser}). There have been a number of advances in unsupervised learning in recent years that seem promising in this regard [Citations].
% There is hope for dispensing with this tradeoff entirely.
% Recent advances in unsupervised learning have offered
% effective tools for summarizing high-dimensional data much akin to relational
% datasets.
% While it was previously thought intractable to approximate the joint data
% distribution of a relation in its full form~\cite{getoor2001selectivity,deshpande2001independence}, {\em deep
%   likelihood models}, a type of statistical density estimator, have
% % enjoyed leaps of progress, achieving
% achieved remarkable success modeling high-dimensional data such as images, text, and audio~\cite{pixelcnn,pixelcnnpp,wavenet, transformer}.
% However, these models only provide {\em point density} estimates (i.e., ``what
% is the likelihood a particular tuple appears in the relation?''), but not {\em
%   range density} estimates that are required by multi-dimensional range
% predicates in virtually every SQL workload (e.g., ``what fraction of tuples have \textsf{price} less
% than \$100 and \textsf{weight} greater than \SI{10}lbs?'').
% Estimating for range queries by summing over all points in the query
% region is prohibitively expensive, given the high-dimensional space a SQL table
% or query typically spans.
% At first glance, although these modern models may provide superior modeling accuracy, %prove a high-fidelity summary,
% % for may provide high precision in
% they appear practically limited to equality predicates for selectivity estimation. An accurate and compact joint approximation would largely dispense with this tradeoff (Figure 1).
% There are well-established techniques in Machine Learning that can be used in this context.
A limitation of these techniques
is that they only address the problem of point density estimation---in query processing terms, they only handle equality predicates.
Full-featured selectivity estimation requires handling not only equality but also range predicates. Estimating the density of a larger subspace requires integrating over that space. In high-dimensional data---e.g., tables with dozens or hundreds of columns---this integration needs to ``roll up'' enormous numbers of potential points: in
a workload we consider, there are $10^{10}$ points in the
region of interest
, which would take more than 1,000 hours to sum over by a
naive enumeration scheme---much longer than scanning the data in the first place.
Range predicate estimation requires new techniques beyond the state of the art.

In this paper, we show how selectivity estimation can be done very accurately at high dimensionality using \emph{deep likelihood models}, which have previously been used successfully for point estimation in domains such as X, Y and Z [cite].
We show how database data---including both numeric and categorical attributes---can be mapped into these models for effective selectivity estimation of equality predicates.
We then introduce a new Monte Carlo integration technique called \emph{progressive sampling}, which leverages the structure of deep likelihood models to produce
very accurate estimation for range queries. By leveraging the availability of conditional probability distributions,
progressive sampling steers the sampler into regions of high probability
density, and then corrects for the induced sampling bias via importance weighting. This extends the state of the art in density estimation generally, with particular applicability to
our problem of general-purpose selectivity estimation.
\jmh{Potentially put some empirical results here. Could be one sentence in this paragraph, or a summary paragraph.}

% they seem limited selectivity estimators at best by
%nly natively supportll-equality queries.
% only natively support estimating all-equality queries, greatly lacking in generality.
% Although the success stories come from images, text or audio,
% relational datasets are amenable.

% our key contribution
% The key contribution of this paper is an algorithm that allows deep likelihood models to handle multi-dimensional range queries, turning these models into general-purpose selectivity estimators.
% In this paper we present 
% The key contribution of this paper is to adapt and extend deep likelihood model-based
% selectivity estimators for selectivity esti, {\em and} an integration technique that
% equips them to efficiently handle multi-dimensional range queries.
% The key contribution of this paper is a technique that allows deep likelihood models to
% handle multi-dimensional range queries, turning them into general-purpose selectivity estimators. \jmh{If this is the key contribution, make that very clear in title and abstract.}

% \jmh{Is this really a relevant metric? What scheme sums over the data space that way?}
% To tackle the sheer scale of typical integration regions found in SQL
% queries,
% To tackle this, %\jmh{our main technical contribution is a new}
% we develop a new Monte Carlo integration technique, termed
% \emph{progressive sampling}, that particularly suits the likelihood
% models under consideration.
%The sampler judiciously navigates the integration region, obtaining rich information from the model as it selects samples.

%The sampler judiciously navigates the integrationregion by consulting the intermediate conditional densities.
% , obtaining rich information using a small amount of samples.Information obtained from one dimension allows the sampler to focus onthe denser sub-region in the next dimension. Each sampled path thus progressivelyzooms in into the smaller, informative parts of the gigantic integration region.
Our technique is effective: it cuts down the estimation latency of the query above to about $10\si{\ms}$.
% cutting the estimation
% thus enhancing any
% off-the-shelf likelihood models of this form to function as a versatile
% selectivity estimator.

% zongheng: consider keeping this here or to Sec:Querying.
% To better understand the hardness of evaluating the integral without progressive
% sampling,
% % in  Figure \ref{fig:uniformvsps} we
% consider a simple relation $R$ with $N$ columns, and with column value distribution skew so that $99\percent$ of the probability mass is contained in the top $1\percent$ of its range. Consider a query with range predicates over the top $50\percent$ of each column. It is easy to see that naive Monte-Carlo integration, which picks random points within the query region, will take on expectation $1/(0.01 / 0.5)^N = 1/0.02^N$ samples to hit within the high-mass region we are integrating over. Therefore, the number of samples required for an accurate selectivity estimate increases exponentially with $N$. Progressive sampling solves this problem by using the factorized model to steer the sampler into the high-mass part of the query region, and then compensating for the induced bias with importance weighting.

% our results
To realize these ideas, we design and implement \sys, %an accurate and practical
a selectivity estimator that approximates the joint data
distribution in its full form, without any column independence assumptions. %jmh{this phrase is redundant by now no? certainly doesn't deserve italics.}
Approximating the joint in full not only provides superior accuracy, but also
frees us
% a database
% an administrator
from specifying what combinations of columns to build synopses on.
% This not only provides superior accuracy, but frees the user from having to worry about defining relation factorizations for performance.
% Our estimator is tailored-made for relational data.
We further propose optimizations to encode and decode a wide spectrum of
characteristics in real-world relational data (e.g., various datatypes, small vs. large domain sizes). Combining our integration
scheme with these practical strategies results in a highly accurate, compact,
and functionality-rich selectivity estimator based on deep likelihood models.
%Training is performed via statistically grounded principles (i.e., maximum likelihood) where no supervised signals or query feedback are required. \jmh{I feel like the unsupervised/data-only approach is an important contribution/philosophy of the paper, and it's kind of buried here.}
%Experimentally, we show that our full joint approximation approach can be used to estimate
%selectivity with state-of-the-art accuracy and are still space- and
%runtime-efficient.

% We demonstrate \sys can learn to capture complex data patterns found in real-world datasets.


% In this paper, we revisit the goal of directly approximating the joint
% distribution in its full form, without any column independence assumption.
% While in the worst case, modeling the joint is no easier than storing the entire
% relation, columns in real datasets are often highly correlated or derived from
% each other (e.g., a functional dependency).  Therefore, there very well might
% exist a substantially lower-dimensional parameterization of the joint
% distribution that is efficient to construct, store, and query.

% Our key idea is to propose using high-capacity deep likelihood models for
% selectivity estimation.  These compact models can capture complex data
% dependencies and avoid the need for hand-specifying distributional relationships.
% Training is performed via statistically grounded principles (maximum
% likelihood) where no supervised signals or query feedback are required.
% Crucially, early in our investigation we realize that a naive adaptation of this
% family of models to the relational setting yields only limited capabilities.
% One of the key technical challenges we have to solve is \emph{efficient
%   integration of point density}, i.e., estimating the amount of density
% contained in a region spanned by \textit{range} predicates.  To tackle the sheer
% scale of typical integration regions, we
% develop a Monte Carlo integration technique, termed \emph{progressive sampling},
% that particularly suits the factorized likelihood models under consideration.
% The sampler judiciously navigates the integration region by consulting the
% intermediate factorized densities, thus enhancing any off-the-shelf likelihood
% models of this form to function as a versatile selectivity estimator.
% % form
% % enhances a vanilla likelihood model to support conjunctions of range
% % predicates over a large number of columns, by navigating
% % that provides factorized
% % conditional densities to efficiently
% % to support
% % We show that a model that only supports point density calculation can be
% % integrated efficiently to answer conjunctions of range predicates over a large
% % number of columns.

%\jmh{OK, now you address data-centric unsupervised head-on. Maybe remove the side-comment above?}
Just like classical synopses, \sys summarizes the data in an unsupervised
fashion.
Training is performed via statistically grounded principles (maximum likelihood) where no supervised signals or query feedback are required.
While many \emph{query-driven} estimators
are concerned with optimizing with respect to a set of training queries
(i.e., ``how much error does the estimator incur on these queries?''),
\sys is optimized with
respect to the underlying data distribution (i.e., ``how divergent is the estimator
from the data?'').
% \jmh{I'd focus on the fact that you kick ass over everything else first. Only after that say that this could also be integrated with query-centric approaches if that proved helpful in those approaches.}
Our direct joint approximation is orthogonal to
query-driven approaches: an unsupervised likelihood model can always take
advantage of additional signals such as query feedback by further fine-tuning.  On the other hand,
being data-driven, \sys supports a much larger set of queries and is automatically robust to query distributional shifts.  Our evaluation
compares \sys to the state-of-the-art unsupervised and supervised techniques, showing \sys to be
the only estimator to achieve \textit{single-digit multiplicative error} at tail for
challenging high-dimensional queries.
% Experimentally, we show that our full joint approximation approach can be used to estimate
% selectivity with superior accuracy when compared against the state-of-the-art, while
% still being space- and
% runtime-efficient.



% Selectivity estimators have always been grounded in statistical estimation
% techniques.  We see \sys as the natural next step of incorporating cross-column
% correlations in a disciplined and scalable fashion.
This paper makes three principal contributions:
\begin{enumerate}
    % \item We motivate the use of deep likelihood models as selectivity
      % estimators (\secref{sec:background}), and propose optimizations
      % to make them
      % suitable for relational datasets (\secref{sec:construction}).
    \item We show how deep likelihood models can be used for selectivity
      estimation (\secref{sec:background}, \secref{sec:likelihood-models}), and develop optimizations
      to make these estimators suitable for relational datasets (\secref{sec:construction}).
    \item We identify range query estimation to be the key challenge for
      likelihood model-based selectivity estimators.  To address this challenge, we propose
      \textit{progressive sampling}, a Monte Carlo integration scheme that
      efficiently estimates range densities even with large query regions (\secref{sec:querying}).
    %   efficiently enhances vanilla deep likelihood models to handle
    % high-dimensional range queries (\secref{sec:querying}).  %We consider this in itself of interest to the machine learning community which has  mostly been concerned with point density.
    \item Our estimator \sys, when evaluated on several real-world datasets
      and compared to baseline of different families (heuristics, real
      DBMSes, statistical methods, supervised learning), achieves
      orders-of-magnitude better accuracy with space usage $\sim 1\%$
      of data size and $\sim 10\si{\ms}$ of estimation latency (\secref{sec:eval}).

% We discuss how \sys can support queries even with a large
% number of range filters, either on base tables or via joins.  We conduct
% comprehensive evaluation to demonstrate \sys's ability to capture complex data
% patterns in real-world datasets, and carefully characterize tradeoffs in
% estimation accuracy, latency, and model construction costs.

\end{enumerate}


==> intro-beforeApr30MorningEdits.tex <==
\section{Introduction}
% what problem, why important, is it unresolved
Estimating the selectivity of a SQL predicate
% is essential
is a core primitive
in query optimization~\cite{systemr}, approximate query processing~\cite{blinkdb}, and performance profiling~\cite{akdere2012learning}.  The main task is to estimate the fraction of a relation that
satisfies a predicate, without actual execution.
% Despite its crucial importance, the problem is widely understood to be unresolved.
Despite its importance, there is wide agreement that the problem is
still unsolved~\cite{leis2015good,leis2018query,reopt}.
Open-source and commercial DBMSes
routinely produce up to $10^4{-}10^8\times$ estimation errors, depending on
the number of attributes, compared to the ground truth~\cite{leis2015good}.

% why is the problem hard
% The problem's hardness comes from the fact that estimators are tasked with condensing information
The fundamental difficulty of selectivity estimation comes from condensing information
about data into summaries~\cite{space_synopsis}.  The predominant approach in database systems today
is to collect single-column summaries (e.g., histograms and sketches) and to
combine these coarse-grained models assuming column independence.  This
represents one extreme, where the summaries are fast to construct and cheap to
store, but compounding errors occur due to the coarse information and over-simplified
independence assumptions.
% On the other extreme, when given access to a complete
% description about data, e.g., the true {\em joint data distribution}, selectivity
% ``estimates'' would be perfect albeit at the cost of intractable construction and
% storage.
On the other end of the spectrum, when given the {\em joint data distribution} of
a relation
(the frequency of each unique tuple normalized by the relation's cardinality),
perfect selectivity ``estimates'' can be read off or computed by integration from the distribution. However,
the {\em joint} is intractable to compute or store for all but the tiniest datasets.
% We show that the intractable joint data distribution of a relation,
 % can be approximated by deep likelihood models
% to a high degree of fidelity while offering compactness, functionality, and
% runtime efficiency.
Thus, traditional selectivity estimators are faced with the hard
tradeoff between the amount of information captured
%(more means better accuracy)
and the cost to construct, store, and query the summary.
%(the more information, the higher the costs).

\begin{figure}[t]
% \centering
\includegraphics[width=0.9\columnwidth]{plots/sol-space.pdf}
% \vspace{.1in}
\caption{Approximating the joint data distribution in full, \sys enjoys high space efficiency and estimation accuracy.\label{fig:teaser}}
\vspace{-.1in}
\end{figure}

% We argue that learning-based approaches can provide access to better points in
% this trade-off space (Figure~\ref{fig:teaser}).
% what enabled our attack
% We argue there is hope for dispensing with this tradeoff entirely.
An accurate and compact {\em joint approximation} would largely dispense with this
tradeoff (Figure~\ref{fig:teaser}).
% There is hope for dispensing with this tradeoff entirely.
Recent advances in unsupervised learning have offered
effective tools for summarizing high-dimensional data much akin to relational
datasets.
While it was previously thought intractable to approximate the joint data
distribution of a relation in its full form~\cite{getoor2001selectivity,deshpande2001independence}, {\em deep
  likelihood models}, a type of statistical density estimator, have
% enjoyed leaps of progress, achieving
achieved remarkable success modeling high-dimensional data such as images, text, and audio~\cite{pixelcnn,pixelcnnpp,wavenet, transformer}.
However, these models only provide {\em point density} estimates (i.e., ``what
is the likelihood a particular tuple appears in the relation?''), but not {\em
  range density} estimates that are required by multi-dimensional range
predicates in virtually every SQL workload (e.g., ``what fraction of tuples have \textsf{price} less
than \$100 and \textsf{weight} greater than \SI{10}lbs?'').
Estimating for range queries by summing over all points in the query
region is prohibitively expensive, given the high-dimensional space a SQL table
or query typically spans.
At first glance, although these modern models may provide superior modeling accuracy, %prove a high-fidelity summary,
% for may provide high precision in
they appear practically limited to equality predicates for selectivity estimation.
% they seem limited selectivity estimators at best by
%nly natively supportll-equality queries.
% only natively support estimating all-equality queries, greatly lacking in generality.
% Although the success stories come from images, text or audio,
% relational datasets are amenable.

% our key contribution
% The key contribution of this paper is an algorithm that allows deep likelihood models to handle multi-dimensional range queries, turning these models into general-purpose selectivity estimators.
The key contribution of this paper is to introduce deep likelihood model-based
selectivity estimators, {\em and} an integration technique that
equips them to efficiently handle multi-dimensional range queries.
% The key contribution of this paper is a technique that allows deep likelihood models to
% handle multi-dimensional range queries, turning them into general-purpose selectivity estimators. \jmh{If this is the key contribution, make that very clear in title and abstract.}
Multi-dimensional query regions are extremely challenging to integrate over: in
a workload we consider, there can be up to $10^{10}$ points in the
region of interest, which would take more than 1,000 hours to sum over by a
naive enumeration scheme---much longer than scanning the data in the first
place.
% \jmh{Is this really a relevant metric? What scheme sums over the data space that way?}
% To tackle the sheer scale of typical integration regions found in SQL
% queries,
To tackle this, %\jmh{our main technical contribution is a new}
we develop a new Monte Carlo integration technique, termed
\emph{progressive sampling}, that particularly suits the likelihood
models under consideration.
%The sampler judiciously navigates the integration region, obtaining rich information from the model as it selects samples.
By leveraging the availability of conditional probability distributions,
progressive sampling steers the sampler into regions of high probability
density, and then corrects for the induced sampling bias via importance weighting.
%The sampler judiciously navigates the integrationregion by consulting the intermediate conditional densities.
% , obtaining rich information using a small amount of samples.Information obtained from one dimension allows the sampler to focus onthe denser sub-region in the next dimension. Each sampled path thus progressivelyzooms in into the smaller, informative parts of the gigantic integration region.
Our technique is effective: it cuts down the estimation latency of the query above to about $10\si{\ms}$.
% cutting the estimation
% thus enhancing any
% off-the-shelf likelihood models of this form to function as a versatile
% selectivity estimator.

% zongheng: consider keeping this here or to Sec:Querying.
% To better understand the hardness of evaluating the integral without progressive
% sampling,
% % in  Figure \ref{fig:uniformvsps} we
% consider a simple relation $R$ with $N$ columns, and with column value distribution skew so that $99\percent$ of the probability mass is contained in the top $1\percent$ of its range. Consider a query with range predicates over the top $50\percent$ of each column. It is easy to see that naive Monte-Carlo integration, which picks random points within the query region, will take on expectation $1/(0.01 / 0.5)^N = 1/0.02^N$ samples to hit within the high-mass region we are integrating over. Therefore, the number of samples required for an accurate selectivity estimate increases exponentially with $N$. Progressive sampling solves this problem by using the factorized model to steer the sampler into the high-mass part of the query region, and then compensating for the induced bias with importance weighting.

% our results
To realize these ideas, we design and implement \sys, %an accurate and practical
a selectivity estimator that approximates the joint data
distribution in its full form, without any column independence assumptions. %jmh{this phrase is redundant by now no? certainly doesn't deserve italics.}
Approximating the joint in full not only provides superior accuracy, but also
frees us
% a database
% an administrator
from specifying what combinations of columns to build synopses on.
% This not only provides superior accuracy, but frees the user from having to worry about defining relation factorizations for performance.
% Our estimator is tailored-made for relational data.
We further propose optimizations to encode and decode a wide spectrum of
characteristics in real-world relational data (e.g., various datatypes, small vs. large domain sizes). Combining our integration
scheme with these practical strategies results in a highly accurate, compact,
and functionality-rich selectivity estimator based on deep likelihood models.
%Training is performed via statistically grounded principles (i.e., maximum likelihood) where no supervised signals or query feedback are required. \jmh{I feel like the unsupervised/data-only approach is an important contribution/philosophy of the paper, and it's kind of buried here.}
%Experimentally, we show that our full joint approximation approach can be used to estimate
%selectivity with state-of-the-art accuracy and are still space- and
%runtime-efficient.

% We demonstrate \sys can learn to capture complex data patterns found in real-world datasets.


% In this paper, we revisit the goal of directly approximating the joint
% distribution in its full form, without any column independence assumption.
% While in the worst case, modeling the joint is no easier than storing the entire
% relation, columns in real datasets are often highly correlated or derived from
% each other (e.g., a functional dependency).  Therefore, there very well might
% exist a substantially lower-dimensional parameterization of the joint
% distribution that is efficient to construct, store, and query.

% Our key idea is to propose using high-capacity deep likelihood models for
% selectivity estimation.  These compact models can capture complex data
% dependencies and avoid the need for hand-specifying distributional relationships.
% Training is performed via statistically grounded principles (maximum
% likelihood) where no supervised signals or query feedback are required.
% Crucially, early in our investigation we realize that a naive adaptation of this
% family of models to the relational setting yields only limited capabilities.
% One of the key technical challenges we have to solve is \emph{efficient
%   integration of point density}, i.e., estimating the amount of density
% contained in a region spanned by \textit{range} predicates.  To tackle the sheer
% scale of typical integration regions, we
% develop a Monte Carlo integration technique, termed \emph{progressive sampling},
% that particularly suits the factorized likelihood models under consideration.
% The sampler judiciously navigates the integration region by consulting the
% intermediate factorized densities, thus enhancing any off-the-shelf likelihood
% models of this form to function as a versatile selectivity estimator.
% % form
% % enhances a vanilla likelihood model to support conjunctions of range
% % predicates over a large number of columns, by navigating
% % that provides factorized
% % conditional densities to efficiently
% % to support
% % We show that a model that only supports point density calculation can be
% % integrated efficiently to answer conjunctions of range predicates over a large
% % number of columns.

%\jmh{OK, now you address data-centric unsupervised head-on. Maybe remove the side-comment above?}
Just like classical synopses, \sys summarizes the data in an unsupervised
fashion.
Training is performed via statistically grounded principles (maximum likelihood) where no supervised signals or query feedback are required.
While many \emph{query-driven} estimators
are concerned with optimizing with respect to a set of training queries
(i.e., ``how much error does the estimator incur on these queries?''),
\sys is optimized with
respect to the underlying data distribution (i.e., ``how divergent is the estimator
from the data?'').
% \jmh{I'd focus on the fact that you kick ass over everything else first. Only after that say that this could also be integrated with query-centric approaches if that proved helpful in those approaches.}
Our direct joint approximation is orthogonal to
query-driven approaches: an unsupervised likelihood model can always take
advantage of additional signals such as query feedback by further fine-tuning.  On the other hand,
being data-driven, \sys supports a much larger set of queries and is automatically robust to query distributional shifts.  Our evaluation
compares \sys to the state-of-the-art unsupervised and supervised techniques, showing \sys to be
the only estimator to achieve \textit{single-digit multiplicative error} at tail for
challenging high-dimensional queries.
% Experimentally, we show that our full joint approximation approach can be used to estimate
% selectivity with superior accuracy when compared against the state-of-the-art, while
% still being space- and
% runtime-efficient.



% Selectivity estimators have always been grounded in statistical estimation
% techniques.  We see \sys as the natural next step of incorporating cross-column
% correlations in a disciplined and scalable fashion.
This paper makes three principal contributions:
\begin{enumerate}
    % \item We motivate the use of deep likelihood models as selectivity
      % estimators (\secref{sec:background}), and propose optimizations
      % to make them
      % suitable for relational datasets (\secref{sec:construction}).
    \item We introduce the use of deep likelihood models as selectivity
      estimators (\secref{sec:background}, \secref{sec:likelihood-models}), and develop optimizations
      to make them suitable for relational datasets (\secref{sec:construction}).
    \item We identify range query estimation to be the key challenge for
      likelihood model-based selectivity estimators.  In response, we propose
      \textit{progressive sampling}, a Monte Carlo integration scheme that
      efficiently estimates range densities even with large query regions (\secref{sec:querying}).
    %   efficiently enhances vanilla deep likelihood models to handle
    % high-dimensional range queries (\secref{sec:querying}).  %We consider this in itself of interest to the machine learning community which has  mostly been concerned with point density.
    \item Our estimator \sys, when evaluated on several real-world datasets
      and compared to baseline of different families (heuristics, real
      DBMSes, statistical methods, supervised learning), achieves
      orders-of-magnitude better accuracy with space usage $\sim 1\%$
      of data size and $\sim 10\si{\ms}$ of estimation latency (\secref{sec:eval}).

% We discuss how \sys can support queries even with a large
% number of range filters, either on base tables or via joins.  We conduct
% comprehensive evaluation to demonstrate \sys's ability to capture complex data
% patterns in real-world datasets, and carefully characterize tradeoffs in
% estimation accuracy, latency, and model construction costs.

\end{enumerate}


==> intro-v0.tex <==
\section{Introduction}
 Cardinality estimator is a central component to any query optimizer.  Its main task is to answer, for a given query, its estimated cardinality or selectivity.  The estimates are fed into the query optimizer to make performance-critical decisions, such as logical join ordering, physical operator selection, scheduling, and resource allocation.  Despite its crucial importance, the problem is widely reported to be unresolved---popular open-source as well as commercial data management systems can routinely produce up to $10^8\times$ estimation errors, compared to ground-truth. 

Casting the problem via a statistical lens, the estimation can be viewed as a \textit{likelihood modeling} problem.  Let us assume a base table with two numerical columns.  To estimate the selectivity for any conjunction of range filters (including equality) on the columns, it is sufficient to have access to \textit{a joint distribution for the table}, namely $P(C_1, C_2)$.  To obtain the selectivity of the query,
$\texttt{sel}(C_1 = 10, C_2 = 7)$, one simply plugs in the literals to look up the probability mass, $P(10, 7)$.  
Range queries as well as querying only a subset of the columns are supported by marginalization.
% Generalization of this scheme to range queries as well as querying only a subset of the columns has also been well-studied in the statistics community.  
Of course, computing or approximating the joint distribution is often computationally expensive or, for anything other than tiny-scale data, intractable. 

The key idea of this paper is to propose \textit{using deep neural net-based likelihood models as cardinality estimators}.  There are several immediate benefits.  First, real-world relational datasets contain an explosive amount of patterns that are impractical to hand-annotate.  These patterns can either exist in the schema (``salary is correlated with age and education, to different degrees''), or in the values (``there is no car with make Honda and model Jetta'').  High-capacity function approximators, e.g., deep nets, are proven capable of learning hidden patterns with remarkable effectiveness.  Second, unlike classical likelihood models such as Bayesian networks, recent advances in deep likelihood models do away with the need to specify (or search for) a good dependency specification between columns.  Instead, we can afford to approximate the joint distribution in its most general form.
For example, company X reports that its typical ``data lake'' contains Y tables in a total of Z columns---specifying a dependency structure at such scale is costly.
Lastly, if one desires a ``personalized'' cardinality estimator that understands the data at hand as much as possible, a high-capacity deep model is exactly the choice for maximally over-fitting to user data.

Building on these observations, we design and implement \sys, an efficient and accurate cardinality estimator based on deep likelihood models. We make the following contributions:
\begin{enumerate}
    \item We show that deep likelihood models can be used to estimate cardinalities with unprecedented accuracy and moderate efficiency.
    \item We discuss how \sys can support queries even with a large amount of range filters, either on base tables or via joins. 
    \item We conduct comprehensive evaluation to carefully characterize tradeoffs in estimation accuracy, latency, and model construction costs.  We include baseline estimators of different types: non-learning, classical learning, and deep learning.
\end{enumerate}


% Since it approximates the joint distribution, likelihood modeling is a direct, statistically grounded approach to cardinality estimation.  The choice of deep net-based models are simply an instantiation of this approach.
% This approach has the following immediate benefits.  First, deep nets learn to detect patterns in data with remarkable effectiveness.  With real-world relational datasets containing a myriad of correlation and anti-correlation, automatic detection of such patterns is essential.  Second, deep likelihood models are high-capacity.  As universal function approximators, they have a much better chance to learn a more accurate likelihood model than classical alternatives (e.g., graphical models).  

==> intro-v1.tex <==
\section{Introduction}
Estimating the selectivity of a SQL query is a core primitive in query
optimization [?], query performance profiling [?], and approximate query
processing [?].  The estimator's main task is to answer, without actual
execution, the fraction of a relation that satisfies a particular predicate.
The predominant approach in database systems today is to collect single-column
summaries (e.g., histograms and sketches) and to combine these coarse models
assuming statistical independence between columns.  Despite its crucial
importance, the problem is widely reported to be unresolved.  Open-source as
well as commercial data management systems can routinely produce up to
$10^8\times$ estimation errors compared to ground-truth~\cite{leis2015good}, due
to coarse-grained summarization and incorrect independence assumptions.

\begin{figure}[htp]
% \centering
\includegraphics[width=0.9\columnwidth]{plots/sol-space.pdf}}
% \vspace{.1in}
\caption{Approximating the joint data distribution in full, \sys enjoys high space efficiency and estimation accuracy.\label{fig:teaser}}
\vspace{-.1in}
\end{figure}

Casting the problem via a statistical lens, the estimation
% can be viewed as a
is fundamentally a
\textit{likelihood modeling} problem.  Let us assume a base table with two
numerical columns.  To estimate the selectivity for any conjunction of range
filters (including equality) on the columns, it is sufficient to have access to
\textit{the joint probability distribution} for the table, namely $P(C_1, C_2)$.
To obtain the selectivity of the query,
% $\texttt{sel}(C_1 = 10, C_2 = 7)$,
$C_1 = 10 \wedge C_2 = 7$,
one
simply plugs in the literals to look up the probability mass, $P(10, 7)$.  Range
queries as well as querying only a subset of the columns are supported by
enumeration.  Of course, computing and storing the joint is intractable since
its full form contains an exponential number of entries.  Instead, prior work
has considered approximating the joint~\cite{getoor2001selectivity,
  deshpande2001independence}.  However, these approaches have historically
suffered from several important pitfalls: (1) for learning and computational
efficiency, certain simplifying assumptions are still made (e.g., conditional
independence between columns), which lead to a loss of approximation accuracy,
(2) hand-specifying or searching for a statistically accurate dependency graph
between columns is expensive, (3) scaling to high-cardinality columns or a large
number of columns is challenging, and (4) querying these approximations for
range predicates is inefficient.

In this paper, we revisit the goal of directly approximating the joint
distribution in its full form, without any column independence assumption.
While in the worst case, modeling the joint is no easier than storing the entire
relation, columns in real datasets are often highly correlated or derived from
each other (e.g., a functional dependency).  Therefore, there very well might
exist a substantially lower-dimensional parameterization of the joint
distribution that is efficient to construct, store, and query.

Our key idea is to propose using high-capacity deep likelihood models for
selectivity estimation.  These (compact) models can capture complex data
dependencies and avoid the need of hand-specifying distributional relationships.
Training is performed via statistically grounded principles---maximum
likelihood---where no supervised signals or query feedback are required.
Crucially, early in our investigation we realize that a naive adaptation of this
family of models to the relational setting yields only limited capabilities.
One of the key technical challenges we have to solve is \emph{efficient
  integration of point density}, i.e., estimating the amount of density
contained in a region spanned by \textit{range} predicates.  To tackle this, we
develop a Monte Carlo integration technique, termed \emph{progressive sampling},
that particularly suits the factorized likelihood models under consideration.
We show that a model that only supports point density calculation can be
integrated efficiently to answer conjunctions of range predicates over a large
number of columns.

Building on this core technical contribution, we design and implement \sys, an
efficient and practical selectivity estimator based on deep likelihood models.
Our adaptations are tailored-made for relational data.  \sys proposes
various encoding and decoding strategies to handle a spectrum of column
characteristics common in real-world data (e.g., small vs. large domain size, or
discrete vs. continuous).  Experimentally, we show that deep likelihood models
can be used to estimate selectivity with state-of-the-art accuracy and are still
space- and runtime-efficient.  We discuss how \sys can support queries even with
a large amount of range filters, either on base tables or via joins. We conduct
comprehensive evaluation to carefully characterize tradeoffs in estimation
accuracy, latency, and model construction costs.

Like classical synopses, \sys learns to understand the data in an unsupervised
fashion. Contrasting the unsupervised regime many \emph{query-driven} techniques
have been proposed in the literature.
% These techniques seek to avoid modeling
% the joint distribution altogether; instead, they assume access to a set of
% ``representative'' queries or tuples to learn and extrapolate from.
These supervised techniques assume access to a set of ``representative'' queries
or tuples to learn and extrapolate from.  Classical histograms have been
augmented with query-driven construction or refinement heuristics (e.g.,
STHoles~\cite{stholes}, ISOMER~\cite{isomer}).  Vanilla kernel density
estimators (KDE) sample a set of tuples at construction time and distribute
density mass within a neighborhood of the samples.  Heimel et
al.~\cite{selectivity-kde} extends vanilla KDEs by optimizing their
performance-critical bandwidth parameter on a set of training queries.  Recent
work by Kipf et al.~\cite{kipf2018learned} breaks grounds in proposing a novel,
set-invariant supervised network for predicting selectivities.  This supervised
learning treatment is really a modern take on exact selectivity estimation [?],
where the exact results from trial queries are fed into a model which then predicts
the selectivities of future queries.  Common to all these approaches is the
premise that the optimization is done with respect to a set of training queries
(``how much error does the estimator incur on these queries?''), not with
respect to the underlying data distribution (``how divergent is the estimator
from the data?'').  Our direct joint approximation is complimentary
to query-driven approaches: a likelihood model trained in an unsupervised
fashion can always take advantage of additional supervised signals by further
fine-tuning.  On the other hand, \sys requires no supervised training data and
hence, vacuously, is robust to query distributional shifts.  Our evaluation
compares \sys to these families of techniques, showing \sys to be
the only estimator to achieve \textit{single-digit multiplicative error} at the maximum for
challenging high-dimensional range queries.

While the role of machine learning in database internals will continue to be
hotly debated, selectivity estimation has, in a sense, always been a machine
learning problem.  This important DBMS component has always taken advantage of
statistical estimation and distributional approximation.  We see \sys as the
natural next step of incorporating cross-column correlations in a statistically
disciplined and scalable fashion.  This paper makes the following contributions
and is organized as follows:
\begin{enumerate}
    \item We motivate why deep likelihood models as selectivity estimators is a natural and versatile choice (\secref{sec:background}).  We propose various optimizations (\secref{sec:construction}) to make the models suitable for relational settings.
    \item We propose \textit{progressive sampling}, a technique that enhances vanilla deep likelihood models to handle
    high-dimensional range queries (\secref{sec:querying}).  We consider this scheme in itself of interest to the machine learning community which has  mostly been concerned with point density.
    \item On several real-world datasets, we conduct evaluation to understand tradeoffs in estimation accuracy, latency, and model construction costs.  When compared to baseline estimators of different types (heuristics, real DBMSes, statistical methods, deep learning), we show that \sys achieves order-of-magnitudes better accuracy while moderately consuming $\sim 1\%$ of data size and $\sim 10\si{\ms}$ query latency (\secref{sec:eval}).
\end{enumerate}



% Building on these observations, we design and implement \sys, an efficient and accurate cardinality estimator based on deep likelihood models. We make the following contributions:
% \begin{enumerate}
%     \item We show that deep likelihood models can be used to estimate cardinalities with unprecedented accuracy and moderate efficiency.
%     \item We discuss how \sys can support queries even with a large amount of range filters, either on base tables or via joins.
%     \item We conduct comprehensive evaluation to carefully characterize tradeoffs in estimation accuracy, latency, and model construction costs.  We include baseline estimators of different types: non-learning, classical learning, and deep learning.
% \end{enumerate}


% Since it approximates the joint distribution, likelihood modeling is a direct, statistically grounded approach to cardinality estimation.  The choice of deep net-based models are simply an instantiation of this approach.
% This approach has the following immediate benefits.  First, deep nets learn to detect patterns in data with remarkable effectiveness.  With real-world relational datasets containing a myriad of correlation and anti-correlation, automatic detection of such patterns is essential.  Second, deep likelihood models are high-capacity.  As universal function approximators, they have a much better chance to learn a more accurate likelihood model than classical alternatives (e.g., graphical models).

==> intro-v2-apr23.tex <==
\section{Introduction}
Estimating the selectivity of a SQL query is a core primitive in query
optimization [?], query performance profiling [?], and approximate query
processing [?].  The estimator's main task is to answer, without actual
execution, the fraction of a relation that satisfies a particular predicate.
The predominant approach in database systems today is to collect single-column
summaries (e.g., histograms and sketches) and to combine these coarse models
assuming statistical independence between columns.  Despite its crucial
importance, the problem is widely reported to be unresolved.  Open-source as
well as commercial data management systems can routinely produce up to
$10^8\times$ estimation errors compared to ground-truth~\cite{leis2015good}, due
to coarse-grained summarization and incorrect independence assumptions.

\begin{figure}[htp]
% \centering
\includegraphics[width=0.9\columnwidth]{plots/sol-space.pdf}}
% \vspace{.1in}
\caption{Approximating the joint data distribution in full, \sys enjoys high space efficiency and estimation accuracy.\label{fig:teaser}}
\vspace{-.1in}
\end{figure}

Casting the problem via a statistical lens, the estimation
% can be viewed as a
is fundamentally a
\textit{likelihood modeling} problem.  Let us assume a base table with two
numerical columns.  To estimate the selectivity for any conjunction of range
filters (including equality) on the columns, it is sufficient to have access to
\textit{the joint probability distribution} for the table, namely $P(C_1, C_2)$.
To obtain the selectivity of the query,
% $\texttt{sel}(C_1 = 10, C_2 = 7)$,
$C_1 = 10 \wedge C_2 = 7$,
one
simply plugs in the literals to look up the probability mass, $P(10, 7)$.
Albeit expensive, range
queries as well as querying only a subset of the columns are supported by
 enumeration, e.g., $P(C_1 < 10, C_2 = \ast) = \sum_{x_1 < 10}\sum_{x_2} P(x_1, x_2)$.  Of course, computing and storing the joint is intractable since
its full form contains an exponential number of entries.  Instead, prior work
has considered approximating the joint~\cite{getoor2001selectivity,
  deshpande2001independence}.  However, these approaches have historically
suffered from several important pitfalls: (1) for learning and computational
efficiency, certain simplifying assumptions are still made (e.g., conditional
independence between columns), which lead to a loss of approximation accuracy,
(2) hand-specifying or searching for a statistically accurate dependency graph
between columns is expensive, (3) scaling to high-cardinality columns or a large
number of columns is challenging, and (4) querying these approximations for
range predicates is inefficient.

In this paper, we revisit the goal of directly approximating the joint
distribution in its full form, without any column independence assumption.
While in the worst case, modeling the joint is no easier than storing the entire
relation, columns in real datasets are often highly correlated or derived from
each other (e.g., a functional dependency).  Therefore, there very well might
exist a substantially lower-dimensional parameterization of the joint
distribution that is efficient to construct, store, and query.

Our key idea is to propose using high-capacity deep likelihood models for
selectivity estimation.  These compact models can capture complex data
dependencies and avoid the need for hand-specifying distributional relationships.
Training is performed via statistically grounded principles (maximum
likelihood) where no supervised signals or query feedback are required.
Crucially, early in our investigation we realize that a naive adaptation of this
family of models to the relational setting yields only limited capabilities.
One of the key technical challenges we have to solve is \emph{efficient
  integration of point density}, i.e., estimating the amount of density
contained in a region spanned by \textit{range} predicates.  To tackle the sheer
scale of typical integration regions, we
develop a Monte Carlo integration technique, termed \emph{progressive sampling},
that particularly suits the factorized likelihood models under consideration.
The sampler judiciously navigates the integration region by consulting the
intermediate factorized densities, thus enhancing any off-the-shelf likelihood
models of this form to function as a versatile selectivity estimator.
% form
% enhances a vanilla likelihood model to support conjunctions of range
% predicates over a large number of columns, by navigating
% that provides factorized
% conditional densities to efficiently
% to support
% We show that a model that only supports point density calculation can be
% integrated efficiently to answer conjunctions of range predicates over a large
% number of columns.

Building on this core technical contribution, we design and implement \sys, an
efficient and practical selectivity estimator based on deep likelihood models.
Our adaptations are tailored-made for relational data.  \sys proposes
various encoding and decoding strategies to handle a spectrum of column
characteristics common in real-world data (e.g., small vs. large domain size, or
discrete vs. continuous).  Experimentally, we show that deep likelihood models
can be used to estimate selectivity with state-of-the-art accuracy and are still
space- and runtime-efficient.  We discuss how \sys can support queries even with
a large number of range filters, either on base tables or via joins. We conduct
comprehensive evaluation to carefully characterize tradeoffs in estimation
accuracy, latency, and model construction costs.

Like classical synopses, \sys learns to understand the data in an unsupervised
fashion. Contrasting the unsupervised regime many \emph{query-driven}, or supervised, techniques
have been proposed in the literature.
% These techniques seek to avoid modeling
% the joint distribution altogether; instead, they assume access to a set of
% ``representative'' queries or tuples to learn and extrapolate from.
These techniques assume access to a set of ``representative'' queries
or tuples to learn and extrapolate from.  Classical histograms have been
augmented with query-driven construction or refinement heuristics (e.g.,
STHoles~\cite{stholes}, ISOMER~\cite{isomer}).  Vanilla kernel density
estimators (KDE) sample a set of tuples at construction time and distribute
density mass within a neighborhood of the samples.  Heimel et
al.~\cite{selectivity-kde} propose query-driven KDEs by optimizing the
performance-critical bandwidth parameter on a set of training queries.  Recent
work by Kipf et al.~\cite{kipf2018learned} breaks grounds in proposing a novel,
set-invariant supervised network as selectivity estimator.  There, exact
selectivities from trial queries combined with a materialized sample are used to
train a model to predict selectivities for future queries.
% This supervised
% learning treatment is really a modern take on exact selectivity estimation [?],
% where the exact results from trial queries are fed into a model which then predicts
% the selectivities of future queries.
Common to all these approaches is the
premise that the optimization is done with respect to a set of training queries
(``how much error does the estimator incur on these queries?''), not with
respect to the underlying data distribution (``how divergent is the estimator
from the data?'').  Our direct joint approximation is complimentary
to query-driven approaches: a likelihood model trained in an unsupervised
fashion can always take advantage of additional supervised signals by further
fine-tuning.  On the other hand, \sys requires no supervised training data and
hence, vacuously, is robust to query distributional shifts.  Our evaluation
compares \sys to these families of techniques, showing \sys to be
the only estimator to achieve \textit{single-digit multiplicative error} at tail for
challenging high-dimensional range queries.

% While the role of machine learning in database internals will continue to be
% hotly debated, selectivity estimation has, in a sense, always been a machine
% learning problem.  This important DBMS component has always taken advantage of
% statistical estimation and distributional approximation.
Selectivity estimators have always been grounded in statistical estimation techniques.  We see \sys as the natural next step of incorporating cross-column correlations in a disciplined and scalable fashion. This paper makes the following contributions and is organized as follows:
\begin{enumerate}
    \item We motivate why deep likelihood models as selectivity estimators is a natural and versatile choice (\secref{sec:background}).  We propose various optimizations (\secref{sec:construction}) to make the models suitable for relational settings.
    \item We propose \textit{progressive sampling}, a technique that enhances vanilla deep likelihood models to handle
    high-dimensional range queries (\secref{sec:querying}).  We consider this scheme in itself of interest to the machine learning community which has  mostly been concerned with point density.
    \item On several real-world datasets, we conduct evaluation to understand tradeoffs in estimation accuracy, latency, and model construction costs.  When compared to baseline estimators of different types (heuristics, real DBMSes, statistical methods, deep learning), we show that \sys achieves order-of-magnitudes better accuracy while moderately consuming $\sim 1\%$ of data size and $\sim 10\si{\ms}$ query latency (\secref{sec:eval}).
\end{enumerate}



% Building on these observations, we design and implement \sys, an efficient and accurate cardinality estimator based on deep likelihood models. We make the following contributions:
% \begin{enumerate}
%     \item We show that deep likelihood models can be used to estimate cardinalities with unprecedented accuracy and moderate efficiency.
%     \item We discuss how \sys can support queries even with a large amount of range filters, either on base tables or via joins. 
%     \item We conduct comprehensive evaluation to carefully characterize tradeoffs in estimation accuracy, latency, and model construction costs.  We include baseline estimators of different types: non-learning, classical learning, and deep learning.
% \end{enumerate}


% Since it approximates the joint distribution, likelihood modeling is a direct, statistically grounded approach to cardinality estimation.  The choice of deep net-based models are simply an instantiation of this approach.
% This approach has the following immediate benefits.  First, deep nets learn to detect patterns in data with remarkable effectiveness.  With real-world relational datasets containing a myriad of correlation and anti-correlation, automatic detection of such patterns is essential.  Second, deep likelihood models are high-capacity.  As universal function approximators, they have a much better chance to learn a more accurate likelihood model than classical alternatives (e.g., graphical models).  

==> revision_cover_letter.tex <==
% https://stackoverflow.com/questions/51337095/latex-one-column-title-and-index-in-a-two-column-document
\twocolumn[
    \begin{@twocolumnfalse}
        \begin{center}
          \ttlfnt Response to Reviewer Comments
         \end{center}
     \end{@twocolumnfalse}
]
We thank our reviewers for their detailed and constructive
feedback.
% \zongheng{say something about we have addressed all.}
% on their thoughtful comments, we have accordingly revised the paper
Over the course of past several months, we have addressed all comments and the
paper has significantly improved as a result.
 In this cover letter, we first respond to major points raised in the meta-review and by multiple reviewers, and then also include detailed responses to individual comments. We use \revision{\textit{blue text}} to denote responses to reviewer
  comments in this letter as well as revised text in the
  main paper.

\section*{Meta-review comments}

\begin{reviewerquote}
{\bf M1.} What is the set of probabilistic
inference queries the model supports? What about the variability of inference runtime?
\end{reviewerquote}
\noindent
\revision{
%We support arbitrary range predicates (in fact, any boolean function over a single column) over arbitrary subsets of columns, as described in~\secref{subsec:problem}.
  \sys supports estimating the cardinality of conjunctions of single-column boolean predicates (e.g., range predicates, IN, and LIKE clauses),
  % conjunction of any boolean function
  % applied to individual column,
  across arbitrary subsets of columns. %, as described in~\secref{subsec:problem}.
  The supported query set is more general than rectangular range predicates with lower and
  upper bounds. For ease of exposition, we use \emph{range} to denote the valid
  set of values a column (correspondingly, a query) can take on.
  We have revised~\secref{subsec:problem} to clarify.

The autoregressive model itself produces point density estimates, which we
augment with progressive sampling
% (i.e., forward sampling with range likelihoods)
to produce range density estimates.
The sampling procedure requires at most \texttt{num\_columns} model forward passes for each query, so the latency is bounded.
%The sampling procedure requires at most \texttt{num\_columns} model forward passes for each query.
%In this revision we have introduced a simple optimization to allow skipping model forward passes on wildcard columns.
\sys estimates queries with fewer columns faster (e.g., median at $\sim 5 \si{\ms}$) and those with more columns in linearly more time (e.g., max at $\sim 10 \si{\ms}$).
% (tail is bounded by $<2\times$ median).
We have correspondingly updated Figure~\ref{fig:latency} and clarified this point in \secref{subsec:latency}.


  % We have clarified this point in \secref{X}.

  % In this
  % revision we have introduced a simple optimization, wildcard-skipping
  % (\secref{sec:wildcard-skipping}), that allows skipping model forward passes on
  % wildcard columns in a query.  We have correspondingly updated the latency CDF
  % (Figruee~\ref{fig:latency-cdf}).  \sys estimates queries with fewer columns
  % faster (e.g., median at $\sim 5 \si{\ms}$) and those with more columns in
  % linearly more time (tail is bounded by $<2\times$ median).

  % It is important
  % to note that the sampling procedure requires the same amount of time
  % regardless of the inference query, since it always executes
  % \texttt{num\_columns} batched forward passes through the model regardless of
  % the query \zongheng{This statement is true for pre-revision; now, with
  %   wildcard-skipping, the latency may be affected a little bit. TODO: investigate?}.
}

\begin{reviewerquote}
{\bf M2.} The paper requires a clear explanation of how their work relates and compares with the work by Uria et al. who has done some work on this problem.
\end{reviewerquote}
\noindent
\revision{
  Uria et al.~\cite{uria13_deep_tract_densit_estim} is work published in the ML
  community and is not concerned with issues that arise in selectivity
  estimation: they do not support range density, and are not concerned with efficient
  inference. %\jmh{Anything else? I took out the vague ``e.g.'' ... if you have other examples, list them.}
  They propose
  % ensembles of NADE models with
  a specific autoregressive architecture (NADE) and train the model
  % \jmh{what is ``it'', the model? I'm slightly confused by the tense of ``trains'' -- this sentences is a little broken}
  simultaneously on different column orderings to handle point queries on different columns.
  % \jmh{The ``different orderings'' is a bit vague .. you mean ordering of columns yes?}
  In contrast, \sys can take any deep autoregressive architecture as a building block
  (e.g., MADE, NADE, or Transformer) and train it on a single order.
  % \jmh{any deep autoregressive architecture as a building block (...) and train a model on a single order.}
  Moreover, \sys's inference procedure supports
  range predicates, unlike Uria et al.
  % , and also executes in constant time
  % irrespective of the inference query \zongheng{revisit this constant-time
  %   claim}.
  Incorporating their \emph{order-agnostic} training is a possible future
  optimization for \sys, though in preliminary experiments we did not find
  the performance benefits on top of progressive sampling significant. We have
  included this discussion in \secref{sec:column-ordering}.}
% \ekl{TODO: clarify this in related work section, and say here we have added this clarification}

\begin{reviewerquote}
 {\bf M3.} What is the effect of the order of the chosen chain model on the set of probabilistic inference queries the model supports, and how this relates to the performance of their sampling algorithm.
\end{reviewerquote}
\noindent
\revision{
 %Thanks for this comment.
%The chosen column order does not affect the set of supported queries.
%As mentioned in our response to M1, we support conjunctions of arbitrary boolean restriction on each column domain.
%Such order-independent marginalization is achieved via progressive sampling.
This is an interesting question, and spurred us to do more experimentation.
The order in which we train the model does not affect the types of queries supported.
However, the order does affect the estimation variance.
We have performed an in-depth study and found that randomly sampled orderings (1) perform consistently well up to and including 99-th percentile error, but (2) can have wildly differing estimation variance in the max error.
%In terms of the impact of ordering on estimation variance, the reviewers rightly pointed out that an in-depth study was missing. %ordering  a significant impact on estimation accuracy.
%We have since performed in-depth studies on how column ordering affects estimation variance. We find that randomly sampled orderings have wildly differing variance in the extreme error tail.
Instead of choosing a random ordering, we found that several sensible heuristic orderings grounded in information theory exhibit low estimation variance across datasets even for the max error.
The detailed evaluation has been added in \secref{eval:variance-reduction} and corresponding discussion in \secref{sec:column-ordering}.

}
  % We analyze the effect of ordering on performance in a newly added section \ekl{TODO should this be a section in the paper instead of a big chunk of the response current in major points?}. It is important to note however that the ordering does not affect the set of inference queries supported. We support any type of range restriction on variables, on arbitrary subsets of variables.}

\begin{reviewerquote}
  {\bf M4.} The paper should evaluate their cardinality estimation algorithm on different attribute combinations to see how it handles marginalization.
\end{reviewerquote}
\noindent
\revision{
  We believe this comment is in error.
  Our evaluation is already on different attribute combination subsets, selected randomly according to the
  procedure described in \secref{sec:eval-workloads}. All generated queries
  contain ranges, do not necessarily follow the model order, and
  require complex marginalization; solving these challenges is the main purpose of the progressive sampling algorithm.}
 %\jmh{if we're apologizing, what are we doing to fix it?}
  %As mentioned in our response to M1, a simple trick now allows
  %the progressive sampler to efficiently marginalize by \emph{not} sampling
  %through wildcards, increasing its efficiency further.}


\begin{reviewerquote}
   {\bf M5.} The paper should present their sampling algorithm as forward sampling, and not importance.
\end{reviewerquote}
\noindent
\revision{
We thank the reviewers for pointing out this connection.  To make the relation to prior work more clear and highlight our delta, we have revised the
presentation of progressive sampling (\secref{sec:prog-sampling})
  to be ``forward sampling with likelihood weighting on ranges''.  Standard
  forward sampling with likelihood weighting requires each
  observed variable be equal to \emph{some specific value}; our
  algorithm is an extension of it to allow each observed variable to be \emph{a
    range of values}. In other words, the former handles point queries, while
  the latter extends the former to handle range queries. %\zongheng{actually modify main text}.

 With regard to terminology, likelihood weighting is indeed a simple form of importance sampling (cf. Koller and Friedman~\cite[Chapter~12]{pgm_textbook}).  To expand, suppose we want to estimate
 \[
\phat(X_1\in R_1) = \mathbb{E}_{x_1 \sim \phat(X_1)}\mathbf{1}[x_1 \in R_1].
\]
Progressive sampling does not draw $x_1$ samples from the target distribution
$\phat(X_1)$.  Instead, it draws from $\phat(X_1 | X_1 \in R_1)$, the proposal distribution in importance
sampling terms.  The importance weight of this $x_1$ sample, thus, is the ratio
\[
  \phat(X_1 = x_1)/\phat(X_1 = x_1 | X_1 \in R_1) = \phat(X_1 \in R_1),
\]
 which is the first term in
Equation~\ref{eq:three-col-progressive}. %\zongheng{TODO: maybe also talk about how progressive sampling is similar to Wander Join~\cite{wander_join}, Index Based Join Sampling~\cite{leis2017cardinality}?}
}

\section*{Points brought up by multiple reviewers}

\begin{reviewerquote}
{What types of predicates does \sys support? (R2, R3)}
\end{reviewerquote}
\noindent
\revision{
  Please see our earlier response to M1 and the revised \secref{subsec:problem}.
  % As noted in the meta-review response and Section \ref{subsec:problem}, we
  % support arbitrary range predicates over arbitrary subsets of columns. To the
  % best of our knowledge the support of range predicates with likelihood models
  % is novel to \sys. To be more specific, any predicate that can be expressed as
  % a conjunction of boolean expression over single column values is supported,
  % which includes equalities, inequalities, IN expressions, etc. We do however
  % require the set of possible column values to be known ahead of time.
}

% \begin{reviewerquote}
% {Can you provide an analysis of the impact of model architecture and hyperparameters? (R1, R2, R4)}
% \end{reviewerquote}
% \noindent
% \revision{
%   We added an analysis of the impact of ResMADE and Transformer architectures in
%   \ekl{Section TODO}.
% % We provide a detailed analysis of these effects and heuristics for selecting effective column orderings.
% }

% \begin{reviewerquote}
% {Can you compare this approach to using Bayesian Networks?}
% \end{reviewerquote}
% \noindent

% \revision{}

\begin{reviewerquote}
  What is the impact of variable ordering on estimation quality? (M3; R2; R4) % (M3; R2A2; R4D2-2)
\end{reviewerquote}
% \revision{
% There are two
% major treatments for ordering in existing neural density estimation literature:
% (1) train with many orders, infer with an order most suitable to the query; (2)
% train and infer with a fixed order.  However, most ML works optimize for the
% model's goodness-of-fit (e.g., in terms of negative log likelihood).
% We investigate how ordering affects our specific task of selectivity estimation in the following steps.

% First, in Section \secref{X} we sample many random orderings for a given schema
% and train a unique \sys model for each ordering.  This experiment questions \emph{how different orderings affect estimation quality}.
% We found that even though different orderings result in similar entropy gaps
% (goodness-of-fit to data), their maximum Q-errors have wildly differing
% variance.  Most random orderings have worse maximum errors than the natural
% schema order.  This finding suggests that if approach (1) above, i.e.,
% ``order-agnostic training'', is adopted, high maximum Q-errors are still hard to
% avoid.  (This statement is about worst-case error of a large 2000-query
% workload.  If we put ourselves to a lower bar, e.g., 99\%-tile error, then all
% orders work well---i.e., about 2x for everyone.  We focus on the max error.)

% Second, we observe that a simple trick can effectively reduce the estimation
% errors even for bad orderings.  Recall that \sys in its pre-revision form treats
% unqueried columns in any query as wildcards, and samples through their full domains just as
% regular, queried columns.  This was a simple treatment to handle arbitrary
% marginalization but was quite inefficient.  A simple trick is now employed:
% during training, we randomly mask a few columns to signal their ``absence'', and
% during estimation, we set unqueried columns to the special per-column
% ``absence'' values, hence they no longer require wasteful sampling.  Section
% \secref{XX} details this trick, and \secref{YY} reports the effect of this
% optimization.  The optimizations of column-masking and
% wildcard-skipping significantly reduced the variance of almost all orders: even many previously ``bad'' random orders are made ``good''.

% Finally, we have found a few heuristically-chosen orderings (based on
%   intuition from information theory) to work well (Section \secref{XX}).  In summary, \sys adopts
%   fixed-order training, and enjoys low (single-digit) max Q-error
%   with natural table order, randomly sampled orders, or heuristic orders under
%   column-masking and wildcard-skipping optimizations.
% }
\noindent
\revision{
  Please see our response to M3; we have added a detailed study in
  \secref{sec:column-ordering} and \secref{eval:variance-reduction}.

% The column ordering used to construct the model significantly affects the
% variance of the estimator leading to potentially higher worst-case errors.  Our
% paper now contains experiments that evaluate randomly-chosen orders
% \sk{reference} against sensible heuristics to advise users how to select these
% orders.  In the process of running these additional experiments and noticing
% particularly poor performance on ``wildcard'' queries, we discovered a simple
% training trick that can mitigate the effects of bad orderings.  During training,
% we randomly mask columns to signal their ``absence'', and during estimation, we
% use a dedicated ``wildcard'' symbol to represent columns that are missing from
% the predicate.  Section \secref{XX} provide details, and \secref{YY} reports the
% effect of this optimization. After this optimization, many previously ``poor''
% random orders have comparable performance to the best orders without this
% optimization.

% Of course, there are treatments for ordering in existing density estimation
% literature---where state-of-the art approaches train the model with many orders,
% infer with an order most suitable to the query. We find that these approaches
% are currently insufficient in a database context and may not scale to the
% dataset sizes and complexity that interest our community.
}

\begin{reviewerquote}
How does \sys handle updates? (R1, R2, R4)
\end{reviewerquote}
\noindent
\revision{
%We currently do not consider updates in \sys \zongheng{Well, we need to weaken this statement or revise the main text's discussion on updates.}.
Thanks for this question.
Similar to other state-of-the-art works~\cite{cardlearner, kipf2018learned} in learning-based estimators, we can periodically
retrain \sys models when a certain amount of updates or appends have accumulated. % when their performance degrades due to insertion and update.
As an optimization, we can use the previous model to warm-start the re-training.
We agree with the reviewers that efficient incremental model update is an
important topic worthy of detailed study, which we defer to future
work.
We have clarified this point in \secref{subsec:overview}.
%However, for re-training (e.g., a new day of data has accumulated into a new partition), the optimization can be sped up by using the previous model to warm-start the training process. We agree with the reviewers that this is an important topic worthy of detailed study, which we defer to future work.
% However, we do believe that
% training is significantly faster if only a small amount of data is changed or
% added and the previous model can be used to warm-start the training process.
% We defer this study to future work.


% We note that update handling is a concern
% shared by many classical synopses \zongheng{Not true; R1 specifically said it's
% very easy to refresh histograms}, and that \sys can leverage system-level techniques for handling updates from the
% literature such as partitioning and periodic incremental / bulk updates, which
% work regardless of the underlying model. For example, in many cases only the
% most recent partition of data is updated, and so you can keep a small model
% frequently retrained for just that partition, and a large model over the full
% dataset. Since \sys only takes a few passes (epochs) over the dataset to train
% the model, the IO cost is not significantly higher than with other bulk
% approaches. \sys does however require a GPU to retrain.
}

\section*{Response to Reviewer 1}
% \zongheng{Accept.}
\begin{reviewerquote}
{\bf D1.} The method presented in this paper seems harder to ``re-train'' when
data has changed.
\end{reviewerquote}
\noindent
\revision{Please see our response to the previous question about how \sys handles updates. Indeed, we agree that this is an
  important future topic for ``machine learning in query
  optimizer'' research.
  % \zongheng{Awkward response?
}

\begin{reviewerquote}
  {\bf D2.} What are strategies to simplify such hyperparameter optimization?
  % How sensitive are deep likelihood models to relations with different number of attributes and cardinalities?
\end{reviewerquote}
\noindent
\revision{
  As Reviewer 1 rightly points out, choosing sensible architectures given a
  specific dataset or task is important for production use.
  % This research area of Auto ML is actively being worked on in the machine learning community.
  For our setting, as a rule of thumb distilled from our evaluation, we suggest \sys to be
  created with a parameter count
  $0.1\%\sim1\%$ of the dataset size.  %Once the parameter count is fixed, one
%  could adopt the standard practice where deeper %networks generally
%  are more expressive than shallow-but-wider networks.
  Moreover, our evaluation now includes
  comparison to several autoregressive building blocks
  (\secref{subsec:model-choice}), and we find that \sys's performance is not overly
  sensitive to the specific autoregressive architecture.
  % MADE and
  % ResMADE to be easy-to-implement and sufficiently high-capacity.
  % have evaluated against several
  % architectures (MADE, ResMADE, Transformer)
  % research area
  % [see meta-review response]
}

\begin{reviewerquote}
 {\bf D3.} Indicate what percentage of time is plan generation versus estimation so the comparison is more meaningful.
\end{reviewerquote}
\noindent
\revision{
  Without modifying the source code of \pg and
  \sqlserv, it seems difficult to isolate the time spent on estimation from the
  rest of the query optimization pass.
  % However, note that the overheads from
  % plan generation should be mostly due to control logic---
  However, since there is no complex
  access paths nor join orders to optimize over in our evaluation setup, any
  extra overheads outside of estimation should be mostly due to control logic.
  % \jmh{Kind of a copout. It's all in a single file,  \texttt{src/backend/optimizer/path/clausesel.c}. You could just trace time spent under the first function in that file, \texttt{clauselist\_selectivity()}.  Easy to instrument that code to track time, or you could just use gprof or the like.}
  }

  % \zongheng{
  %   TODO? Is this a reasonable question?}}

\section*{Response to Reviewer 2}
% \zongheng{TODO: address we remove RelNet}

% \zongheng{Weak Accept. Hard-core old-school graphical model person.  Lots of requests.}

\begin{reviewerquote}
{\bf W1.} Broad claims on novelty that are not correct.
\end{reviewerquote}
\noindent
\revision{
  We apologize for not clearly stating the connection between standard forward sampling and progressive sampling.
  As in our response to M5, the novelty of our estimation problem comes from the need to estimate
  range cardinalities, for which prior methods were insufficient.
  With regard to methods, standard forward
  sampling does not perform likelihood weighting; moreover, standard forward
  sampling \emph{with} likelihood weighting assumes singleton values for the
  observed variables.  Progressive sampling is an extension of the latter algorithm to
  support ranges of values for the observed variables.
  We have clarified these connections and distinctions in \secref{sec:prog-sampling}, and we
  believe this strengthens the paper and puts its contributions into better context.
%\zongheng{Is this sufficient for R2's ``The proposed sampling or model are not new.'' claim? I think R2 is bothered by progressive sampling. In ``additional thoughts'', he said ``The authors should clearly state why they believe it is novel and not just an instance of forward sampling.'' \zongheng{Joe suggested reiterating we are not direct application. }}
  % We support the specification of ranges of observations (range predicates),
  % which to the best of our knowledge is novel.
}

\begin{reviewerquote}
{\bf W2.} No comparison against state-of-the-art density estimators from the ML community.
\end{reviewerquote}
\noindent
\revision{
  % \zongheng{Joe suggested responding to what he suggested.}
  Thanks for raising this point.  We have now implemented and compared to two advanced
  deep autoregressive models.  ResMADE~\cite{resmade} is a recent extension to Masked Autoencoder that
  adds residual connections to facilitate information
  flow. Transformer~\cite{transformer} is an autoregressive model
  responsible for an array of recent state-of-the-art advances in language modeling
  tasks~\cite{bert,xlnet,gpt2}.  We found that, at similar parameter count,
  (1) Transformer and ResMADE do achieve better entropy gaps (KL divergence from
  data) than MADE, due to superior information aggregation (self-attention) and better information flow (residual connections), respectively;
  (2) however, the more advanced models do not yield consistently better
  estimation errors.
  We added the analysis of these architectures to
  \secref{subsec:model-choice} and Table~\ref{table:ar-choice}.

  Overall, \sys takes any deep autoregressive model as its building block.  It
  uses this model as a subroutine by invoking forward passes. Progressive
  sampling equips such a subroutine to estimate range density.

  % The \sys architecture is compatible with any autoregressive density
  % estimator. Our main contribution is extending it to support range predicates
  % during inference. With respect to model use, we use MADE, which is a more
  % efficient variation of estimators such as NADE used in Uria et al. In
  % Section TODO we also compare against newly proposed ResMADE and Transformer
  % architectures, but do not find a significant performance improvement.
}


\begin{reviewerquote}
{\bf W3.} The use of the masked auto encoder and how it is mentioned is off (see
Section 4.3)
\end{reviewerquote}
\noindent
\revision{
  % \zongheng{What is this comment talking about?  How about we respond by: }
  We have revised \secref{subsec:model-choice} to point out that (1) \sys allows any
  autoregressive model to be plugged in, and (2) we now have three models from
  the ML literature to compare between, MADE, ResMADE, and Transformer.
  % We primarily use this straw man architecture to illustrate how auto-regressive
  % estimators can be logically constructed. In practice, we use the more
  % efficient MADE architecture. For clarity, we will remove this un-used
  % architecture from the final paper since we now evaluate against ResMADE and
  % Transformer.
}

\begin{reviewerquote}
{\bf D1 (comparison to directed models).} The proposed method is as simple as
approximating a conditional probability table (CPT) with a neural network. A CPT
is a function hence all that is being solved here is a regression problem over
complex CPTs.
The authors need to state this clearly in their manuscript so that their work is put
in the right context... It is surprising that the authors do not compare against
the methods (or a simplified version of the methods) presented in [39]. I was
expecting a comparison against a graphical model approach, where one estimates
the structure from the data and then fits the model parameters. The authors
should extend their manuscript with this comparison.
\end{reviewerquote}
\noindent
% \zongheng{we also need to address the first part of this complaint.}
\revision{Indeed, the two approaches referred to in
this comment are also based on unsupervised joint approximation just like \sys.
We have chosen two representatives of these families: the
\textsf{MaxDiff(V,A)} histogram discussed by Poosala et al.~\cite{poosala1997selectivity}, as well as a Bayes net
estimator based on Chow-Liu trees~\cite{chowliu} (we chose this structure since
empirically it gave the best results for the allowed space).
% , when all estimators are subject to the same storage budget we set,
We found that \maxdiff's accuracy is limited by its partitioning heuristics and the uniform
spread assumption.
As a result, both the 99-th percentile error and the max error are more than two orders-of-magnitude worse than \sys.
For BN, its CPT sizes scale with the cube of column domain
sizes, so we opted to use equal-frequency discretization to keep space under budget.
We found that BN provides considerably
better estimates than \maxdiff and is competitive with supervised approaches. However, in our experiments the \sys model still outperforms BN, since it requires neither conditional independence assumptions nor lossy discretization.
% % , but still falls short of the top-of-the-pack
% presumably thanks to its use of conditional independence assumptions.
The results have been correspondingly updated into the evaluation section (\secref{sec:eval}).


Reviewer 2 also rightly points out that autoregressive density estimation has
close connections to ``regression problem over complex CPTs''.
% However, we wish to point out that this
% line of research in ML has not traditionally adopted this
% regression viewpoint---likely because such a
This viewpoint requires carefully
defining ``regression'' (e.g., making sure the outputs lie on the probability
simplex).  The task has been more thought of as classification
or language modeling in the neural density estimation literature, which,
by definition, implies emitting a probability distribution over a domain.
Lastly, \sys is not a graphical-NN hybrid. \sys uses a single, standalone deep likelihood model to approximate the full joint distribution.
% We have clarified this in \secref{XX}. \zongheng{where?}

% We added this to our evaluation in \ekl{Section TODO}. Since Bayesian networks
% do not support range predicate inference out of the box, we applied the same
% progressive sampling procedure to both \sys and a Bayes Net. This ensures a fair
% comparison between the use of deep likelihood models and traditional bayesian
% network approach.
% We use a Chow-Liu tree as the Bayesian Network,  Since the size of conditional probability tables scales with the cube of column cardinalities, we use equal-frequency discretization to bound the space consumption and inference cost.

% Overall we found that while the bayesian network approach worked well, it was significantly outperformed by the full \sys model due to the removal of the need for discretization and any conditional independence assumptions.

}

\begin{reviewerquote}
  {\bf D2 (comparison between different autoregressive models).}
  % TODO: copy-pasta.
\end{reviewerquote}
\noindent
\revision{
  Please see our response to W2.  We thank Reviewer 2 for the pointers to Rippel
  \etal~\cite{rippel2013high} and Inouye \etal~\cite{inouye18a}; we have opted to include new evaluation on ResMADE and
  Transformer for the following reasons.
  % Rippel \etal~predates the three architectures we include by a few years.
  The three architectures we chose are newer than Rippel \etal~by a few years and are in wide use.
  The core contribution of Inouye \etal~appears to be an \emph{abstract} (quoting the authors) algorithmic framework that logically subsumes several types of generative
  models, not just deep autoregressive ones.
  % Further, its central building
  % block is based on \emph{invertible flows}, while the autoregressive models
  % \sys uses need not be flows.
  To test whether \sys is sensitive to the
  predictive performance of the underlying model, we believe Transformer is
  a sufficiently advanced architecture for the task---considering that it underpins many of the recent breakthroughs in natural language processing.

  % Thanks for this comment.
  % We added an analysis of the impact of ResMADE and Transformer architectures in \secref{X}.
  }

\begin{reviewerquote}
{\bf D3.1.} The authors claim that their method is ``automatically robust to query distributional shifts'' . How is this the case given that their method fits the empirical distribution of the data?
\end{reviewerquote}
\noindent
\revision{
  % The empirical distribution of the data does not change with respect to
  % the query workload.
  By robustness to \textit{query} distributional shifts, we
  meant that users are free to submit any valid queries on the data, once a model is
  trained.
  The training
  procedure does not assume any query workload distribution. (An analogy would
  be after a classical histogram is constructed, it can be used to estimate any
  queries that it supports.)

  % Note that we are claiming robustness to \textit{query} distributional shifts
  % (i.e., new predicates submitted by the user), not \textit{data} shifts (which
  % could require retraining).
}

\begin{reviewerquote}
{\bf D3.2.} How does one go about handling insertions in your model and specifically how do you handle out of domain values? A small discussion will benefit the paper.
\end{reviewerquote}
\noindent
\revision{
For updates, please see our response to ``How does Naru handle updates? (R1, R2, R4)''.

With respect to handling queries with out-of-domain values (no change in the data),
% it can answer such queries
simple query rewrite can be used to map them to their respective domains.
As an example, suppose $\textsf{year}$'s domain is $\{ 2017, 2019 \}$.  A range
query with an out-of-domain literal, say ``$\textsf{year} < 2018$'', can be
rewritten as ``$\textsf{year} \leq 2017$'' such that the literal falls within
the domain.  The correct substitution values are found by inspecting the
(assumed to be known) domain.
For equality queries with out-of-domain literals, \sys simply returns a
cardinality of 0.  We have clarified this in \secref{sec:querying}.
  % We have clarified this in \zongheng{todo}.
  % \zongheng{don't see any natural place to add this out-of-domain
  %   discussion. one issue is parsing/processing, the other issue is staleness.}
}

\begin{reviewerquote}
{\bf D3.3.} You need to provide more details on how discretization is performed and what is its effect on your method.
\end{reviewerquote}
\noindent
\revision{
% \jmh{When I hear the word "discretization" I think of lossy transformations. Do we want to say up front that we do not do any lossy discretizing, we simply map categorical values into a numeric domain?}
  Thanks for pointing this out.  Indeed, the word ``discretization'' was
  confusing.  \sys simply uses a standard dictionary encoding scheme for preprocessing.
  % As described in \secref{sec:encoding-decoding}, we use order-preserving
  % dictionary-encoding for discretization.  It is a lossless transformation.
  For a column domain $A_i$, the encoding is a bijection between $A_i$ and
  $[0, |A_i|)$.  The order for each column is the natural order associated with that
  datatype (e.g., alphabetical ordering for strings, numerical ordering for
  numerics/dates).  Thus, it is an order-preserving, lossless transformation. We have revised \secref{sec:encoding-decoding} to clarify this point.
  % This translation map is lossless. %does not lose information.
  % Discretization was not necessary for the datasets we used, since the
  % model overhead is linear in the cardinality of the columns (unlike Bayes
  % Nets), and the datasets had a most tens of thousands of unique values per
  % column. For larger column cardinalities (i.e., in the millions of values), we
  % are exploring factorization of variables into multiple sub-variables (e.g.,
  % lower bits and upper bits). Since this topic is not well addressed by the deep
  % learning literature \zongheng{Not true? Byte pair encoding.}, we believe a
  % detailed analysis of factorization strategies for continuous and large-value
  % discrete variables is a good topic for future work.
}

\begin{reviewerquote}
{\bf D3.4.} You need to provide some examples on the queries you consider to be out-of-distribution. Section 6.3 does not provide the necessary details to the reader.
\end{reviewerquote}
\noindent
% \jmh{The reviewer is asking for examples. You're just re-explaining. That's kind of not helpful. Can't you give a short example in the text?}
% \zongheng{I can't think of an example query that is meaningful.  It would just
%   look like an in-distribution query.  It really depends on what the literals
%   are drawn from (so looking at the literals won't help).}
\revision{As \secref{subsec:ood} describes, an out-of-distribution query is one whose
  literals are drawn randomly from the \emph{domain}, without regard to the
  empirical data.
  An in-distribution query uniformly draws a tuple from the \emph{data} first,
  thus ensuring the literals in that tuple have appeared at least once.
  % This
  % distinction is meant to stress test query-driven supervised methods, and
  % does not matter to data-driven unsupervised approaches like \sys.
  This distinction has also appeared in related work~\cite{selectivity-kde}.
  % We consider it out of distribution if the number of predicates
  % is different from the training set. Note that this is only relevant for
  % supervised models, since \sys sees no queries at training
  % time. \zongheng{Revise this response.}
}

\begin{reviewerquote}
{\bf D3.5.} How is your progressive sampling method different than forward sampling in directed graphical models?
\end{reviewerquote}
\noindent
\revision{
  Please see our responses to M5 and W1.
  % \sys extends forward sampling to support range restrictions on variables.
}

\begin{reviewerquote}
{\bf D3.6.} You need to state that the encoding and decoding cases described in 4.2 are standard. %There is nothing interesting there the moment you describe you are simply solving a regression problem over a CPT.
\end{reviewerquote}
\noindent
\revision{
  Agreed.  We have in fact stated this (``The
  ML community has proposed many such strategies before; we make sensible
  choices by keeping in mind a few characteristics specific to relational
  datasets'').
  % Techniques such as embedding-reuse, to the best of our
  % knowledge, only appear in recent NLP literature for large-scale vocabularies.
  % \jmh{How do you propose to satisfy the reviewer here?}
}


\begin{reviewerquote}
{\bf D3.7.} Your encoding does not take $O(h)$ space. It takes $O(|A|\cdot h)$ space where $|A|$ is the number of distinct values in your domain.
\end{reviewerquote}
\noindent
\revision{Yes, we have indeed pointed out the
  per-column embedding matrix is of this size (``a learnable embedding matrix of type
  $\mathbb{R}^{|A_i| \times h}$'').  $O(h)$ refers to the space a specific
  attribute value
  takes up in the input vector.}

\begin{reviewerquote}
{\bf D3.8.} You need to provide examples of the queries you used and provide more details on the range queries considered.
\end{reviewerquote}
\noindent
\revision{
  Thanks for the suggestion.  We have added an example query in \secref{sec:eval-workloads}.
  % An example random \dmv query is, ``$({\sf fuel\_type}=\text{GAS}) \land ({\sf rev\_ind} = \text{N}) \land ({\sf sco\_ind} = \text{N}) \land ({\sf valid\_date} \geq \text{2018-03-23}) \land ({\sf color} = \text{BK})$''.  We have
  % added this to the evaluation section.
}
% \ekl{yeah we should add one}


\begin{reviewerquote}
{\bf D3.9.} In the intro you talk about <> and IN operators. In your evaluation you talk about =, <=, and >= . You need to fix inaccurate statements.
\end{reviewerquote}
\noindent
\revision{
  % They are equivalent, since you can use a conjunctions and disjunctions of
  % inequalities to implement any of the above.
  In general, we support any conjunction of {single-column boolean
    predicates} (see response to M1).  We have revised \secref{subsec:problem}
  to clarify this point.  For evaluation setup, we generated
  queries with $=, \leq, \geq$ operators for simplicity and consistency with
  prior work~\cite{kipf2018learned}.  We expect related operators (e.g.,
  two-sided ranges) to have identical trends in results since the inference
  algorithm only takes valid regions $\{R_i\}$ as input---what comparison operators
  generated the valid regions do not matter to the sampler.
}

\begin{reviewerquote}
{\bf D3.10.} In Section 2.1 you state that one needs to store CPTs as tables and hence the storage complexity grows for a large number of attributes. There are other methods (such as decision diagrams) that are used beyond tables and do not require storing all possible attribute-value combinations. Especially in your case many of the entries will be zero since you make a closed-world assumption, hence more efficient methods can be used. Be clear about the true storage requirements.
\end{reviewerquote}
\noindent
\revision{Thanks for this insight. Indeed, by making the
  closed-world assumption, the theoretic joint size of a relation $T$ is, in practice,
  bounded by $|T|$, the number of unique tuples in the relation. On top of this, efficient
  storage methods can be further applied.   We have revised \secref{sec:joint-approx}
  to reflect these facts.}

% \begin{reviewerquote}
% {\bf A1.} It is very hard for me to see why progressive sampling is different than forward sampling. By taking the chain rule you have a complex Directed Graphical Model and you then fit the complex conditional distributions using a deep net. please comment on the above.
% \end{reviewerquote}
% \noindent
% \revision{As noted earlier, \sys extends forward sampling to support range restrictions on variables.}

% \begin{reviewerquote}
% {\bf A2.} You need to study the effect that the order of variables has during inference (i.e., when you are estimating marginals for different attribute combinations). A detailed study there is needed (i.e., do not just follow the order in the queries or the order in the table but demonstrate the sensitivity of your method to the order of attributes).
% \end{reviewerquote}
% \noindent
% \revision{TODO.}


\section*{Response to Reviewer 3}
\begin{reviewerquote}
{\bf D1 (form of supported queries: limited or general).} The conditional
distributions...only allow for providing
estimates when the point values to be estimated are of the form $X_1=x_1,\dots,X_i=x_i$
(i.e., a prefix of the predefined order). If this is not the case then
marginalization is required, making the approach very inefficient... There is
no mention of this issue in the paper, and the result is presented as providing
a solution of predicate estimation in general.
\end{reviewerquote}
\noindent
\revision{The supported query set under our formulation is general---please see
  our response in M1.  Moreover, the inference algorithm we propose, progressive
  sampling, handles arbitrary marginalization (please see response to M4). Our evaluation shows that despite
  needing to marginalize arbitrarily, our sampler is efficient under a wide
  selectivity spectrum and is highly accurate (single-digit max error).}

\begin{reviewerquote}
{\bf D2 (difficulty of range density integration; necessity of approximate
inference).} The authors claim that in order to estimate the selectivity of
range queries they need to aggregate over an exponential number of points, but
this is not true because the summations distribute over the conditional
distributions... This is precisely the principle behind inference algorithms in
graphical models... This calls into question the justification for
``progressive sampling'' which is simply forward sampling on a chain Bayesian
network. Importance sampling refers to the case where the evidence is
diagnostic, and is not the case considered in the paper.
\end{reviewerquote}
\noindent
\revision{\sys's formulation factorizes the
  joint distribution using the product (chain) rule, but the resulting model is
  not a simple chain graphical model.  The chosen construction has the logical structure
  that each node $i$ has all nodes with indices $<i$ as its parents---unlike a chain
  where each (non-root) node has a single parent. Hence, an exponential number
  of points is indeed required for exact inference (e.g., consider the very last conditional
  distribution, $\phat(A_n | A_1, \cdots, A_{n - 1})$, which has size
  $O(\prod_{i = 1}^{n - 1}|A_i|)$).

  In terms of interpretation of progressive sampling, please
  refer to our responses to M5 and R2W1.
 % Abbeel: ``note that the range is the observation variable (effectively) in our
 % case; hence the need for likelihood weighting (which is a simple form of
 % importance sampling)''
}


\section*{Response to Reviewer 4}
%\begin{reviewerquote}
%{\bf W1.} The main technical contribution "progressive sampling" is not studied in depth.
%\end{reviewerquote}
%\noindent

%\begin{reviewerquote}
%{\bf W2.} Indeed, how to apply machine learning techniques properly in this problem could be one contribution of this paper, but there are a few more options that can be examined in more depth (e.g. at least experimentally)
%\end{reviewerquote}
%\noindent
%\revision{TODO.}


%\begin{reviewerquote}
%{\bf W3.} Some important issues (e.g., updates) are not discussed in depth
%\end{reviewerquote}
%\noindent
%\revision{TODO.}

\begin{reviewerquote}
{\bf D1.} Can you compare uniform sampling and progressive sampling?
\end{reviewerquote}
\begin{table}[hp]\centering \small%
\ra{1.3}
\begin{tabular}{@{} l l l l l @{}} \toprule
\textsc{Estimator} &  Median  & 95th & 99th & Max \\ \midrule
% Uniform Sampling (no w.s.) &  {$10^4$ } & {$10^6$}  & {$10^6$}  & {$10^7$}  \\

% usample_2000_0_0.570 max 9409313.0 99th 3086041.5516666663 95th 152993.4686363636 median 97.3673062488325
% Uniform Sampling &  {97} & {$1 \cdot 10^5$}  & {$3\cdot 10^6$}  & {$9 \cdot 10^6$}   \\
% usample_2000_0_0.570 max 10520434.0 99th 5459212.419999997 95th 2013608.1499999992 median 3495.5
Uniform Sampling &  {$3 \cdot 10^3$} & {$2 \cdot 10^6$}  & {$5\cdot 10^6$}  & {$1 \cdot 10^7$}   \\

Progressive Sampling &  {1.01} & {1.22}  & {2.00}  & {8.00}  \\
\bottomrule
\end{tabular}
\vspace{0.25em}
\caption{\small{Estimation errors of \sys with uniform sampling vs. \sys with
    progressive sampling on \dmv.  The progressive sampling data is
    the same as Table~\ref{table:standalone-combined}'s \sys-2000; the
    same 2000-query workload is run.}\label{table:unif-vs-prog}}
% \vspace{-0.6cm}
\end{table}
\noindent
\revision{
  In \secref{sec:prog-sampling} we have touched on how uniform sampling
  {had the worst errors among all baselines}, due to its high variance and
  inability to hit non-zero density regions (``To understand the failure mode of uniform sampling...It had the worst errors among
all baselines in our evaluation.'').  We provide the
experimental data in Table~\ref{table:unif-vs-prog} above (due to space
constraint, we have omitted it from the main paper). Over
56\% queries are estimated to have a density of zero; for the remaining queries
severe underestimates are also produced.

% For this run, it
% failed to hit non-zero density samples for over 56\% of queries (and for the
% rest, high errors occur).

}

\begin{reviewerquote}
{\bf D2-2.} There are a number ways to order the attributes but the table order is picked. Do different orderings affect the end-to-end model accuracy? If yes, how to find the right one. If no, why (analytically or experimentally)?
\end{reviewerquote}
\noindent
\revision{Thanks for raising this point.  As noted in our response to M3, we have conducted in-depth studies on the effect of ordering on
  performance in a newly added section and performed analyses on good
  information-theoretic orders.}

\begin{reviewerquote}
{\bf D3.} Handling updates, especially deletes or appending after a long time. There are systematical ways to handle updates in histogram or sample based solutions which does not apply here. Is this a fundamental difficulty for deep learning based solutions? It is fine to say yes, but the discussion in Section 4.1 is too vague.
\end{reviewerquote}
\noindent
\revision{Please see our response to ``How does Naru
  handle updates? (R1, R2, R4)''.  The challenge of continual learning
is actively being researched in the ML community and seems to be fundamentally
difficult~\cite{kirkpatrick2017overcoming}.  As such, we expect systems-level techniques such as efficient
re-training are more pertinent to our immediate needs.}

\begin{reviewerquote}
{\bf D4.} Can progressive sampling be applied in other learning based approaches?
\end{reviewerquote}
\noindent
\revision{Yes, in our extended evaluation we have indeed applied it to Bayesian
  Networks.
  % (though it does not match the performance of
  % deep likelihood models).
  The inference procedure is applicable to any methods that provide access to
  (estimated) conditional distributions $\phat(X_i | x_0, \dots, x_{i-1})$.}

% LocalWords:  subsec autoregressive num Uria et al NADE th eval prog Koller BN
% LocalWords:  hyperparameter dataset ResMADE Autoencoder CPT CPTs MaxDiff Liu
% LocalWords:  Poosala discretization lossy NN Rippel Inouye Naru bijection ood
% LocalWords:  numerics NLP

